Geometry-Oblivious FMM for Compressing Dense SPD Matrices

We present GOFMM (geometry-oblivious FMM), a novel method that creates a hierarchical low-rank approximation, "compression," of an arbitrary dense symmetric positive definite (SPD) matrix. For many applications, GOFMM enables an approximate matrix-vector multiplication in $N \log N$ or even $N$ time, where $N$ is the matrix size. Compression requires $N \log N$ storage and work. In general, our scheme belongs to the family of hierarchical matrix approximation methods. In particular, it generalizes the fast multipole method (FMM) to a purely algebraic setting by only requiring the ability to sample matrix entries. Neither geometric information (i.e., point coordinates) nor knowledge of how the matrix entries have been generated is required, thus the term "geometry-oblivious." Also, we introduce a shared-memory parallel scheme for hierarchical matrix computations that reduces synchronization barriers. We present results on the Intel Knights Landing and Haswell architectures, and on the NVIDIA Pascal architecture for a variety of matrices.

==> comparison.tex <==
%\begin{table}
%\input{tables/otherSoftware.tex}
%\caption{Classical HSS. $N=16384$, $m=512$, $nRhs=1024$, $tol=1e-6$. HODLR: Partial pivoted LU, STRUMPACK: Randomized sampling and ID. Applied to initial ordering. \\  For K03 bug in STRUMPACK: No clear fix. Intel MKL ERROR as sgemms are called with compression rank 0.}
%\end{table}
%Here we show that many cases require a fast method with direct evaluations (and geometry-free sampling) rather than a pure hierarchical semi-separability (hss) approach. 
There exist a few software packages on hierarchical off-diagonal low-rank
matrices. HODLR \cite{ambikasaran2013mathcal} \& STRUMPACK
\cite{rouet-li-e16} 
can be applied black-box on stored matrices and in the explicit matrix version assume that given ordering allows hierarchical semi-separability (hss). Here, we are only interested in the compression and evaluation methods (but both codes also offer factorization). We compared it to our method that only requires access to entries $K_{ij}$.

For compression, HODLR uses a partial pivoted LU decomposition for off-diagonal blocks; STRUMPACK uses a randomized interpolative decomposition according to \cite{liberty2007randomized}. The user may specify random vectors for sampling, but in many cases this is unknown; we used a black-box compression routine using a uniform random distribution and a householder rank-revealing QR. Results for a few interesting cases are listed in table \ref{tab:existingSoftware}; in some of them notable differences occur. K04 is a Gaussian kernel and K07 a Laplace kernel for Gaussian random points; the applied ordering is random and STRUMPACK can lead to very inaccurate results. 

\begin{table}
\input{tables/otherSoftware2.tex}
\caption{ Matrix sizes $N\times N$: For K02-12 $N=36K$, K17 $N=32K$, G03 $N=65K$; leaf node size $m=512$, for evaluation nRhs=$1024$. Internal parameters reasonably adapted such that target error accuracy of around $1E-4$ is reached. 
Results in single precision computed on a Intel Haswell node with 24 cores, 2.6 GHz, 64 GB DDR4-2133.\\
NOTE TO US: \\
STRUMPACK needs some adaption: K04 \& K07 are kernels for gaussian random points, so ordering very random. Larger sampling sizes up to 8192 don't resolve. For K17 and G03 bigger sampling sizes are less accurate }
\label{tab:existingSoftware}
\end{table}


==> hier.tex <==
% Hierarchical matrices can be seen as algebraic generalizations of 
% the FMM where a matrix is compressed using both low-rank and sparse representations
% hierarchically ~\cite{bebendorf08}. 
% We consider a matrix $K\in \mathbb{R}^{N\times N}$ to be
% \emph{hierarchical} if it can be approximated as
% \begin{equation}
%   \label{e:partitioning}
%   \sk{K} =
% \begin{bmatrix}
% K_{\lc\lc} & 0 \\ 
% 0 & K_{\rc\rc} \\ 
% \end{bmatrix} + 
% \begin{bmatrix} 
%   0 & UV_{\lc\rc} \\ 
%   UV_{\rc\lc} & 0 \\ 
% \end{bmatrix} +
% \begin{bmatrix} 
% 0 & S_{\lc\rc} \\ 
% S_{\rc\lc} & 0 \\ 
% \end{bmatrix}
% \end{equation} 
% where the \emph{off-diagonal} blocks $K_{\lc\rc}$ and $K_{\rc\lc}$ 
% are \emph{approximated} by some low-rank factorizations
% $UV$ plus a sparse correction matrix $S$, and
% the \emph{on-diagonal} blocks $K_{\lc\lc}$ and $K_{\rc\rc}$ are
% themselves hierarchical.
% For example, on the right side of \figref{fig:tree}, 
% the sparsity of $S$ is in blue, and $UV$ contains
% many submatrices with different low-rank approximations in pink.
% %For simplicity, we write th approximation as $K\approx \sk{K}=D+UV+S$, 
% %where $UV$ are \emph{far} (approximation), $S$ is \emph{near} (no approximation)
% %and $D$ is again hierarchical.
% 
% %Note that the low-rank plus sparse structure is \emph{not
% %invariant} on permutations, it very strongly depends on the ordering
% %of the columns (or rows since the matrix is symmetric).
% 
% \begin{figure}[h]
%   \centering
%   \includegraphics[scale=.3]{figures/nearfar.pdf}
%   \caption{A hierarchical low-rank plus sparse matrix (right) and 
%     its tree representation.
%     The off-diagonal blocks are combinations of low-rank matrices (pink)
%     and sparse matrices (blue). The on-diagonal blocks are further
%     partitioned as two child nodes in the tree.
%     The $\bigstar$ symbols denote the entries (neighbors) that cannot
%     be approximated.
%     \algref{a:nearnear} computes the sparse pattern  in blue.
%     The low-rank pattern in pink is computed by \algref{a:nearfar}
%     and \algref{a:farfar} with a preorder and postorder traversal.
%     The solid edges in the tree show the traversing paths of
%     \texttt{NearFar($\beta$,0)}. The preorder traversal stops and add
%     $\alpha$ to $Far(\beta)$,
%     because $K_{\beta\alpha}$ does not contain any $\bigstar$.
%     \algref{a:farfar} merges common codes from two children's Far lists.
%     For example, after \texttt{NearFar(\lc,0)} and \texttt{NearFar(\rc,0)},
%     $Far(\lc)=\{\rc,4,4\}$ and $Far(\rc)=\{\lc,4,2\}$.
%     The common nodes will then be removed and merged to their parent such that 
%     $Near(\alpha)=\{4,2\}$, 
%     $Near(\lc)=\{\rc\}$ and
%     $Near(\rc)=\{\lc\}$.
%   }
%   \label{fig:tree}
% \end{figure}
% 
% 
% 
% 
% \textbf{Treecodes.}
% Note that the low-rank structure strongly depends on the ordering
% of the columns (or rows since the matrix is symmetric).
% Such ordering is typically exploited by a geometric tree structure, and
% equation \eqref{fig:tree} resembles the relation between a parent
% node $\alpha$ and the two children $\lc$ and $\rc$ in a tree.
% In \figref{fig:tree},
% a pair of treenodes $\alpha$ and $\beta$ correspond to a submatrix
% $K_{\beta\alpha} = \{K_{ij}\lvert i\in{\beta},j\in{\alpha}\}$.
% To create such approximation in \figref{fig:tree} for each
% $K_{\beta\alpha}$, we need to decide whether $\alpha$ and $\beta$
% are \emph{near} (in blue, cannot approximate) or \emph{far} 
% (in pink, prunable) from each other.
% %from the root to the leaf level.
% 
% \begin{algorithm}[!t]
% \caption{{} \texttt{NearNear}()}
% \begin{algorithmic}
%   \STATE \texttt{\bf for each} $\alpha$ and $\beta$ is leaf \texttt{\bf do}
%   \STATE \gap \texttt{\bf if} $\alpha \cap \MA{N}(\beta)$ \texttt{\bf then}
%            $Near(\beta) = Near(\beta) \cup \alpha$;
% \end{algorithmic}
% \label{a:nearnear}
% \end{algorithm}
% 
% \begin{algorithm}[!t]
% \caption{{} \texttt{NearFar}($\beta$, $\alpha$)}
% \begin{algorithmic}
%   \STATE \texttt{\bf if} $\alpha \cap Near(\beta)$ \texttt{\bf then}
%   \texttt{NearFar}($\beta$,\lc); \texttt{NearFar}($\beta$,\rc); 
%   \STATE \texttt{\bf else} $Far(\beta) = Far(\beta) \cup \alpha$;
% \end{algorithmic}
% \label{a:nearfar}
% \end{algorithm}
% 
% \begin{algorithm}[!t]
% \caption{{} \texttt{FarFar}($\alpha$)}
% \begin{algorithmic}
%   \STATE \texttt{FarFar}($\lc$); \texttt{FarFar}($\rc$);
%   %\STATE \texttt{\bf if} $\alpha$ is not leaf \texttt{\bf then}
%   \STATE $Far(\alpha) = Far(\lc) \cap Far(\rc)$; 
%   \STATE $Far(\lc) = Far(\lc) \backslash Far(\alpha)$; $Far(\rc) = Far(\rc) \backslash Far(\alpha)$;
% \end{algorithmic}
% \label{a:farfar}
% \end{algorithm}
% 
% \textbf{Near-far pruning.}
% Let $\MA{N}(\beta)$ be the set of \emph{neighbors} of $\beta$ ($\beta$ itself and indices 
% shown as $\bigstar$ in \figref{fig:tree}).
% We say $\beta$ and $\alpha$ are \emph{near} if $\alpha \cap \MA{N}(\beta)$ 
% is not empty (i.e., $K_{\beta\alpha}$ contains a least one $\bigstar$).
% \algref{a:nearnear} shows how we construct a list of leaf nodes
% $Near(\beta)$ to denote the non-prunable submatrices (blue) in
% \figref{fig:tree}. Here $Near(\beta) = \{\mu, \beta\}$, because $\mu$ 
% contains a neighbor of $\beta$.
% The prunable submatrices (pink) are
% identified with a preorder and postorder traversal in \algref{a:nearfar}
% and \algref{a:farfar} (see the caption of \figref{fig:tree} for examples). 
% For each leaf node $\beta$, \algref{a:nearfar}
% traverses the tree from the root. 
% If $\alpha \notin Near(\beta)$, then we add $\alpha$ into $Far(\beta)$.
% Otherwise, we recurse to the two children of $\alpha$ to see
% if we can add $\lc$ or $\rc$ to $Far(\beta)$.
% %In \figref{fig:tree}, the solid edges denote the path 
% %of \texttt{NearFar($\beta$,0)}.
% %The traversal stops at $\alpha$, 
% %because $\alpha$ is not in $Near(\beta)$. 
% %On the other hands, $Near(\beta) \in \beta \subset$ node 4; thus the
% %traversal continues after visiting node 4.
% Once we have a prunable list $Far(\beta)$ for each leaf node, 
% \algref{a:farfar} traverses bottom-up to merge the common nodes
% from two children lists $Far(\lc)$ and $Far(\rc)$.
% These common nodes are removed from the children and added to 
% their parent's prunable list $Far(\alpha)$, which
% creates larger pink submatrices.
% %For example, after \texttt{NearFar(\lc,0)} and \texttt{NearFar(\rc,0)},
% %$Near(\lc)=\{\rc,4,4\}$ and $Near(\rc)=\{\lc,4,2\}$.
% %The common nodes will then be removed and merged to their parent such that 
% %$Near(\alpha)=\{4,2\}$, 
% %$Near(\lc)=\{\rc\}$ and
% %$Near(\rc)=\{\lc\}$.
% The number of these blue and pink submatrices are usually linear in $N$.
% If the size (for blue) and the rank (for pink) of these submatrices 
% are also constant in $N$, then matrix-vector multiplication may only require
% $\MA{O(N)}$ work with the following scheme.
% 
% \textbf{Fast multiplication.}
% The key for FMM to reach linear time multiplication is to
% compress a pink $K_{\beta\alpha}$ on both sides 
% using nested column and row bases.
% Here 
% we use a two-sided nested Interpolative Decomposition (ID) to
% approximate $UV_{\lc\rc}$ as
% $P_{\sk{\lc}\lc}^{T}K_{\sk{\lc}\sk{\rc}}P_{\sk{\rc}\rc}$.
% Given $\sk{\lc} \subset \lc$
% and $\sk{\rc} \subset \rc$, $K_{\sk{\lc}\sk{\rc}}$ denotes a submatrix
% of $K_{\lc\rc}$, and $P_{\sk{\lc}\lc}$, $P_{\sk{\rc}\rc}$ are
% matrices of coefficients used to interpolate other entries.
% For an inner node $\alpha$, its skeleton
% $\sk{\alpha} \subset \sk{\lc} \cup \sk{\rc}$ is subselected from its
% children's skeletons. With this nested basis, the parent 
% coefficient matrix $P_{\sk{\alpha}\alpha}$ can be computed as a
% linear combination of two children's coefficients as shown in the box
% \begin{equation}
% \sk{w}_{\alpha} = 
% \framebox[1.1\width]{
% $P_{\sk{\alpha}\alpha}$
% }w_{\alpha}
% =
% \framebox[1.1\width]{$
% P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}
% \begin{bmatrix}
%   P_{\sk{\lc}\lc} & \\
%                   & P_{\sk{\rc}\rc} \\
% \end{bmatrix}
% $}
% \begin{bmatrix}
% w_{\lc} \\
% w_{\rc} \\
% \end{bmatrix}=
% P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}
% \begin{bmatrix}
%   \sk{w}_{\lc} \\
%   \sk{w}_{\rc} \\
% \end{bmatrix}
% \label{e:telescope}
% \end{equation}
% While multiplying weight $w$ from the right, \eqref{e:telescope}
% allows us to compute
% the skeleton weights $\sk{w}_{\alpha}$ for all $\alpha$ in 
% linear time with a postorder traversal (\emph{telescoping}). 
% If we assume there is only a linear number of submatrices $K_{\beta\alpha}$, then
% accumulating the approximate sum for each node $\beta$ as
% \begin{equation}
%   \sk{u}_{\beta} = 
%   \sum_{\alpha \in Far(\beta)} K_{\sk{\beta}\sk{\alpha}}
%   \sk{w}_{\alpha} = 
%   \sum_{\alpha \in Far(\beta)} K_{\sk{\beta}\sk{\alpha}}
%   P_{\sk{\alpha}\alpha}
% \end{equation}
% takes linear time. Similarly, we can apply the same \emph{telescoping} 
% relation from the left (preorder) such that all skeleton potentials 
% \begin{equation}
%   \begin{bmatrix}
%     \sk{u}_l \\
%     \sk{u}_r \\
%   \end{bmatrix} +=
% \framebox[1.1\width]{$
% \begin{bmatrix}
%   P_{\sk{\lc}\lc} & \\
%                   & P_{\sk{\rc}\rc} \\
% \end{bmatrix}^{T}
% P_{\sk{\beta}[\sk{\lc}\sk{\rc}]}^{T}
% $}
% \sk{u}_{\beta}
% \end{equation}
% can also be computed in linear time. Finally, we assume that
% the size of $Near(\beta)$ is constant for each leaf node.
% Then computing $u_{\beta} = \sk{u}_{\beta} + \sum_{\alpha \in
% Near(\beta)}K_{\beta\alpha}w_{\alpha}$ for all leaf node $\beta$
% can also be done in linear tme.
% 
% Overall, FMM assumes that $Near(\alpha)$ and $Far(\alpha)$ 
% are both $\MA{O}(1)$ and uses nested basis on both sides to achieve
% linear time complexity.
% For hierarchical partitioning directly derived from the geometric space, this 
% near-far pruning may be straight forward.
% However, so far we have not yet defined the neighbors 
% ($\bigstar$) and how to partition $K$ as a tree for an arbitrary 
% SPD matrix. 
% In \secref{s:seq}, we illustrate an idea that generalizes this
% near-far pruning to general SPD matrices using the Gramian vector space.


==> hierarchical.tex <==
%Given $N^2$ entries in a dense system matrix it seems to be unavoidable to construct algorithms of complexity less than $\mathcal{O}(N^2)$; for several application problems [insert cites], however, low rank approximations can be applied to some blocks in the matrix. 
%For several application problems a suitable hierarchical subdivision structure can be found by a spatial tree in the physical problem domain ; in high-dimensions ASKIT... make use of randomized projection trees. 


Kernel summation methods - be it analytic, semi-analytic or algebraic - usually compute low rank approximations based on the far-field in the physical problem domain. Analytic and semi-analytic approaches fail in high dimensions as the number of required check and seed points grow exponentially.
In many applications (e.g. data analysis) the high dimensional feature space can be reduced to a low intrinsic dimension; for such kernel summations an algebraic skeletonization-based approach using a randomized projection tree has been introduced \cite{march-xiao-yu-biros15}. Near- and Far-Field separation is based on euclidean neighbor information; i.e. the near iteraction of each row $K_{i:}$ is defined by the
neighbor entries $\MA{N}_i$, and the far interaction is 
computed based on a nested binary partition of $K$.

Any symmetric positive-definite (SPD) matrix can be described as a Gramian matrix of some set of vectors $\phi$.
Given a matrix $K$ (e.g. from a kernel function) being symmetric positive definite, we can assume that there exists a set of vectors $\phi_i \in \mathcal{V}$ which define this matrix by a scalar product,  $$K_{ij}=\mathcal{K} (x_i,x_j)=<\phi_i,\phi_j>$$ 
%short version
%We consider a given symmetric positive-definite (SPD)  matrix $K$ in terms of an underlying Gramian set of vectors as  $$K_{ij}=\mathcal{K} (x_i,x_j)=<\phi_i,\phi_j>$$ 

%Note that we do 	not have direct access to the underlying vector set of $\phi_i$, but only to the scalar product between each other.

Hence, we use the Gramian space in defining a hierarchical subdivision where entries $i$,$j$ are considered near in terms of 
\begin{itemize}
\item[a.] the $L_2$ distance $\norm{\phi_i-\phi_j}_2^2=K_{ii}+K_{jj}-2K_{ij}$
\item[b.] the spanned angle $\sphericalangle(\phi_i,\phi_j)=arccos(\frac{K_{ij}}{K_{ii}K{jj}})$
\end{itemize}

This tree-like partition permutes $K$ into a hierarchical matrix whose off-diagonal blocks are potentially low-rank.
%We first define distance metrics for each column and row based on the symmetric factorization of $K$.

For doing so, we consider a direction spanned by the two farthest points $\phi_\alpha$ and $\phi_\beta$ and split indices $i$ binary by
\begin{itemize}
\item[a.] a $L_2$ based splitting $<\phi_i,\phi_\alpha-\phi_\beta>$
\item[b.] a $d-1$-dimensional two-fold cone spanned in direction $\phi_\alpha-\phi_\beta$, and its opposite direction $\phi_\beta-\phi_\alpha$, i.e. \\ $\frac{1}{\norm{\phi_i}}\norm{<\phi_i,\phi_\alpha-\phi_\beta>}$
\end{itemize}



==> rebuttal.tex <==
We are truly grateful to the reviewers for their time and their extensive and helpful comments. We will try to address all their detailed comments in the final paper. 

---SEVERAL REVIEWERS---

>Why not MPI and DISTRIBUTED ALGORITHMS?

First, we believe that there is no space for this discussion in this paper. 
GOFMM is a completely new algorithm and implementation. Thus, we needed to
demonstrate correctness and single node performance. We tested several
matrices from machine learning, graphs, partial differential equations and
inverse problems; tested different problem sizes; and compared 
Haswell, KNL, and GPU architectures. 
We also demonstrated GOFMM's unique capabilities
(lines 94--96) and addressed the ``permuting problem'' for dense matrices (lines 160--164).  
So we believe this material is enough for an SC paper. 
Several reviewers mentioned that the paper is already too dense.

Second, the MPI extension requires new algorithms, which require a separate paper.  We are currently working on the MPI version of GOFMM.   The basic philosophy of MPI parallelism follows [31] and [43].  New challenges include parallelizing matrix access, integrating the task-scheduling with MPI, 
accounting for off-node dependencies from other ranks, and load-balancing. 
Inter-process job stealing may result in extra communication. 

---REVIEWER 1---

>Specialization of ASKIT.

GOFMM is not a specialization of ASKIT, but rather a generalization.
GOFMM can be applied to an arbitrary SPD matrix, while ASKIT only applies to kernel matrices. ASKIT requires *point coordinates* and a *kernel function* as inputs. Distances are defined using point coordinates, and matrix entries are computed by applying the kernel function to pairs of points. GOFMM only requires the ability to sample entries of the matrix, which is not necessarily a kernel matrix. GOFMM also supports kernel matrices with arbitrary dimensions of data points, like ASKIT. Our examples include such matrices (K04-K10).

>WHY...WRITE YOUR OWN SCHEDULER?

We do so to remove non-standard software dependencies for improving portability and usability. 
GOFMM only requires C++11, OpenMP-3.0, and BLAS/LAPACK.
Our scheduler does not use "omp task". Workers are implemented using "omp parallel for" with static thread binding.

>RUN THE CODE SERIALLY

We can add the results in the revision (space permitting).
Here we report the single core performance of matrix K02 on HASWELL.
Compression takes 9.6 seconds, and evaluation takes 2.8 seconds (54 GFLOPS).

>HYPER-THREADING AND VECTORIZATION ON KNL

Vectors: We do use vectorization throughout.
The computations in Table 2 invoke Intel MKL's BLAS/LAPACK routines,
which use AVX512. (The peak of MKL's GEMM on KNL is about 70\%.)
Our neighbor-search is also highly optimized as  described in [46] and uses vectorization. 

Threads: Hyperthreading is a good idea if we have sufficient tasks. But in GOFMM, we don't have that many tasks. In certain phases of GOFMM, we even assign more than one physical core to a single task when there are not enough tasks.

Performance: The problem sizes of GEMM in GOFMM vary due to the adaptive scheme
(see footnote 4), and many of them are measured to less than 20\% of the GEMM's theoretical peak.

---REVIEWER 2---

>DISTRIBUTED
Please see above.


---REVIEWER 3---

>EXPAND...IN THE CONTEXT OF HOW HPC HARDWARE IS TRENDING TO BEING

Indeed, due to very different kinds of tasks, GOFMM may require
both high throughput (GPU and KNL) and low latency (CPU) units
to be efficient.  Your questions are excellent but we don't have a short answer.  There are several algorithmic opportunities to push GOFMM further into the  high-throughput regime.   We will revise the conclusions to discuss as much as space permits.

>DISCUSSION OF THE RELEVANCE

Please see lines 65-70. Significant applications will be in ML and
fast solvers. We will revise conclusions to add more examples.

>DISTRIBUTED 
Please see above. 

---REVIEWER 4---

>SOFTWARE VERSIONS

Please see lines 910-917.

>NEAREST NEIGHBORS

80\% and 10 iterations are chosen empirically. 
In our experiments, we found that more accurate nearest neighbors do not improve
the GOFMM approximation.  The reason is that the neighbors are used for sampling and selecting groups of direct evaluations between leaves. 
Typically even smaller values are sufficient (70\%).  We use 80\% to be conservative.  More specifically, nearest-neighbors provide a guess of important matrix entries,  which are used in importance sampling and selecting near interactions. According to [32], whether neighbors can improve the accuracy depends on the data (gram-vectors) in different scales.
Typically, neighbor-pruning works better if the intrinsic dimensionality
of the data is low. Consequently, random projection based ANN methods 
also converge faster [43]. Otherwise, it is likely that
neighbors won't improve the accuracy too much.




==> results_ooc.tex <==

%\begin{table}
%\setlength\tabcolsep{2.5pt}
%\centering
%{
%  \begin{tabular}{|>{\columncolor[gray]{0.8}} r|r|rr|rr|rrr|} 
%  \hline
%  \rowcolor[gray]{0.8}
%  dataset & N & $s$ & $\kappa$ & $\%K$ & $\epsilon_2$ & ANN & Skel & Eval \\
%  \hline
%  \textbf{Poisson Problem} & 16k & 512 & 4 & 0.33 & 8.2E-6 & 3 & 2.6 & 0.1 \\
%   & 65k &&& 0.12& 1.5E-4 & 13  & 9 & 0.5 \\
%  \hline
%  \textbf{Helmholtz operator} & 16k & 512 & 4 & 0.35 & 1.2E-5 & 3 & 2.6 & 0.1 \\
%   & 65k &&&-&-& - & - & -\\
%  \hline
%  \textbf{Gauss kernel (10d)} & 16k & 512 & 4 & 1.0 & 1.2E-5 & 3  & 1.5 & 0.2 \\
%   & 65k &&& 0.93& 1.3E-5& 12 & 5.5 & 8.5 \\
%  \hline
%  \textbf{2d var. coef. Poisson} & 16k & 512 & 4 & 0.44 & 2.2E-4 & 3 & 2.4 & 0.1 \\
%  & 65k  &&& 0.9& 2.6E-4& 12 & 9 & 0.25 \\
%  \hline
%  \textbf{2d adv-diff}& 16k  & 512 & 4 & 0.32& 7.4E-1 & 3  & 1.3 & 0.1 \\     & 65k  &&&0.16& 1.8E-1& 12 & 4 & 0.8 \\
%  \hline
%   \textbf{2d react-adv-diff}& 16k  & 512 & 4 & 0.36 & 6.1E-1 & 3 & 1.4 & 0.1 \\
%   & 65k  &&& 0.16 & 3E-1& 12 & 3.6 & 0.8 \\
%   \hline
%  \end{tabular}
%}
%\caption{Single precision datasets with $m = 1,024$, $\tau=0.001$, nrhs=16. Time in seconds on Han. For last two obviously accuracy problems. We can discuss what to show in the table. Helmholtz 65k will be fixed asap. Still in-core, working on OOC
%}
%\end{table}


 \begin{table}
 \input{tables/dense_pointdist_hss.tex}
 \caption{Point $\ell^2$ distances. $N = 16384, m = 1024, \kappa=1, s = 512, nrhs = 512$.}
  \end{table}

 \begin{table}
 \input{tables/dense_kerneldist_hss.tex}
 \caption{Kernel $\ell^2$ distances. $N = 16384, m = 1024, \kappa=1, s = 512, nrhs = 512$.}
  \end{table}

 \begin{table}
 \input{tables/dense_angle_hss.tex}
 \caption{Kernel angles. $N = 16384, m = 1024, \kappa=1, s = 512, nrhs = 512$.}
  \end{table}





 \begin{table}
 \input{tables/dense_pointdist_k16.tex}
 \caption{Point $\ell^2$ distances. $N = 16384, m = 32, \kappa=16, s = 512, nrhs = 512$.}
  \end{table}

 \begin{table}
 \input{tables/dense_kerneldist_k16.tex}
 \caption{Kernel $\ell^2$ distances. $N = 16384, m = 32, \kappa=16, s = 512, nrhs = 512$.}
  \end{table}

 \begin{table}
 \input{tables/dense_angle_k16.tex}
 \caption{Kernel angles. $N = 16384, m = 32, \kappa=16, s = 512, nrhs = 512$.}
  \end{table}





 \begin{table}
 \input{tables/dense_pointdist_budget1.tex}
 \caption{Point $\ell^2$ distances. $N = 16384, m = 32, \kappa=16, s = 512, nrhs = 512, budget = 1\%$.}
  \end{table}

 \begin{table}
 \input{tables/dense_kerneldist_budget1.tex}
 \caption{Kernel $\ell^2$ distances. $N = 16384, m = 32, \kappa=16, s = 512, nrhs = 512, budget = 1\%$.}
  \end{table}

 \begin{table}
 \input{tables/dense_angle_budget1.tex}
 \caption{Kernel angles. $N = 16384, m = 32, \kappa=16, s = 512, nrhs = 512, budget = 1\%$.}
  \end{table}



==> results_sparse.tex <==

\begin{table}[!t]
\setlength\tabcolsep{4.8pt}
\centering
{
  \begin{tabular}{|r|>{\columncolor[gray]{0.8}}r|rr|rr|rrr|} 
  \hline
  \rowcolor[gray]{0.8}
  \# & dataset & $s$ & $\kappa$ & $\%K$ & $\epsilon_2$ & Tree & Skel & Eval \\
  \hline
  & \textbf{inline1} & 512 & 4 & & 7E-16 & 12 & 96 & 39 \\
  & \texttt{GFLOPS} &&&&& - & 69 & 282 \\
  \hline
  & \textbf{msdoor} & 512 & 4 & & 4E-16 &  9 & 75 & 219 \\
  & \texttt{GFLOPS} &&&&& - & 72 & 261 \\
  \hline
  & \textbf{ca-AstroPh} & 512 & 4 & & 1E-16 & $<1$  & 5 & 1 \\
  & \texttt{GFLOPS} &&&&& - & 48 & 340 \\
  \hline
  & \textbf{email-Enron} & 512 & 4 & & 2E-16 & $<1$  & 6 & 4 \\
  & \texttt{GFLOPS} &&&&& - & 44 & 393 \\
  \hline
  \end{tabular}
}
\caption{Sparse datasets with $m = 1,024$, $\tau=0.001$. \texttt{GFLOPS}
  are kind of low. I suspect that the time goes to getting $K_{ij}$
  with the CSC format.
}
\end{table}


==> review.tex <==
---REVIEWER 1---

Summary and High Level Discussion
Authors describe an algebraic variant of FMM (GOFMM) where geometry
information is not needed. The distance metric in the absence of geometric
coordinates is the Gram distance calculated from a set of unknown vectors that
come from the Gramian matrix. 
Strength of the papers: 
1- Very elaborate implementation of the method, and detailed analysis of
complexity.
2- Solid literature review and clear narrative of contributions.
3- Steps to reproduce results were mentioned in the appendix. 

Weaknesses of the paper:
1- Sometimes paragraphs are incoherent and hard to follow. Lots of
proofreading needs to be done.
2- No elaborate comparison of multicore and manycore archs. although there are
strong claims about share memory optimizations made in the contributions.

Comments for Rebuttal
1- This looks like a specialization of (ASKIT: An Efficient, Parallel Library
    for High-Dimensional Kernel Summations). You use specific distance
measures, i.e, gram distance and angle. But ASKIT relaxes the distance
measure (using statistical measures) and supports higher dimensions. So what
are the key advantages of your method over ASKIT besides performance?

2- It's known that omp tasks are not favorable to task-based parallelism, and
there's plenty of DAG based runtime schedulers, e.g. StarPU, Ompss? Why did
you have to write your own scheduler?

3- On KNL and Haswell experiments, why didn't you run the code serially on a
single core? Why did you not utilize the hyperthreads of KNL (68 x 2 and 68 x
    4) to support the claims made about the strength of your DAG-based
scheduler. 
Also, since you are using KNL chips, it is not possible to achieve the
desired floating point performance without using the vector units. I didn't
see that in the current work or in the future work. You are getting a maximum
of around 1000 Gflops, which is 1/6 of the maximum single precision peak.

Detailed Comments for Authors
1- The paper has serious readability issue with many incoherent fragments. 
2- Very tedious background and introduction. Literature review and
background sections should be merged for example. 
3- Details from previous algorithm are mentioned in text, like
near-far-pruning. This could've been avoided by just making brief references
to literature. 
3- In Figure 1, you have the same figure twice with/without log scale.
4- In Figure 6, the same experiments need to be done for HSS and GOFMM.
Currently the experiments look misaligned. If this is not possible
otherwise, a clear explanation should be given on why this is not the case.
5- The captions under the figures are long and distracting. They should be
at most 3 lines, and all the text should go to the body. 
6- A lot of vague abbreviations are used in the text, although explained.
It's very hard to remember things like s, g, m, the ones used in the
experiments sections.

---REVIEWER 2---

Summary and High Level Discussion
The paper presents a fast multipole method for compression of dense symmetric
positive definite matrices that does not rely on apriori knowledge of the
underlying graph. The approach is sound, however, there is no discussion on
applicability of the approach on a distributed memory environment.

Comments for Rebuttal
There is no mention of the extension of this method to a distributed
environment.

Detailed Comments for Authors
Overall: The paper presents a fast multipole method for compression of dense
symmetric positive definite matrices that does not rely on apriori knowledge
of the underlying graph. The approach is sound, however, there is no
discussion on applicability of the approach on a distributed memory
environment.

Strength: The presentation is clear and the approach is solid.

Insufficiency: There is no mention of the extension of this method to a
distributed environment.

Some of the plots are hard to read. For example, in Figure 1, the order of
the entries in the legend should match the order of the lines in the plot.
This would improve readability and make it easier to match a line to a
legend entry. Also, in Figure 5, there is no concept of continuity when
working with discrete matrix examples, hence, why are the entries connected
with lines. A bar graph of some wort would be better suited here.

---REVIEWER 3---

Summary and High Level Discussion
This paper considers using the fast multi-pole method as a tool for the
compression of black-box SPD matrices. The authors compare their approach
against similar libraries, albeit using slightly different algorithms.

While the paper has good use of figures to illustrate the discussed
algorithms, some of the details of the algorithms employed are unclearly
written, e.g., the algorithmic description is extremely dense, with a lot of
details that makes it a bit of a challenge to fully understand the algorithm
(certainly at first pass). Disappointing to see no application to a
distributed setting.

Comments for Rebuttal
At the end of section 4, there is the comment that no one architecture is
suitable for the algorithm, since it contains both extremely parallel and
serial portions. Can the authors expand this discussion in the context of how
HPC hardware is trending to being increasingly parallel. Will this pose
problems, e.g., in the Exascale, if there is a lack of serial processing
performance. Is there a minimum about serial processing throughput required
in order to ensure the algorithm is efficient. For example a minimum CPU to
GPU ratio or in the case of more homogenous architecture, a maximum vector
size that the algorithm will tolerate. 

The conclusion is relatively weak and simply sums up the paper in a couple of
sentences and decribes future objectives. I would like to see a discussion of
the relevance of this algorithm, and similar algorithms in the future. What
makes these algorithms attractive for computational science? Will the
techniques propsed in the paper have increased relevance in computational
science?

Detailed Comments for Authors
Just a comment that the poor strong scaling seen may be caused by NUMA
issues on the Haswell dual socket system, and memory coherence issues on
KNL. It is likely that significantly improved performance would be observed
if MPI was used on both platforms (2-way and 4-way on Haswell and KNL
    respectively).

---REVIEWER 4---

Summary and High Level Discussion
This paper proposes a new method to compress dense symmetric positive definite
(SPD) matrices. A fast multipole method is generalized to only require
sampling matrix entries. A shared-memory implementation is provided, with
results on 22 different matrices on several different architectures.
Strengths:
Good, consistent terminology is used throughout the paper.
A variety of matrices are analyzed on a range of (well-described) hardware
systems.
Weaknesses:
The paper is quite dense, especially in Section 2.
Occasionally there are sentence fragments and other grammatical issues that
distract from the content.

Comments for Rebuttal
What versions of software were used?
In the index nearest neighbor list (lines 297-305), why were 80% accuracy and
10 iterations chosen as stopping criteria?

Detailed Comments for Authors
Line 172 re-orders the sum in equation 1; please be consistent.
Lines 609-629: does s refer to seconds or max. rank (or both)? For instance,
line 616 reports 0.9s in compression.
Tables 3 and 4 may benefit by bold-facing the best results in each row.
The many different experiments run are well organized in the charts, with
good analysis provided.
Table 5 claims to provide efficiency results in GFLOPS; generally,
efficiency is a percentage of peak performance.




==> seq.tex <==
% To transform the high level discussion of near-far pruning into algorithms, 
% we separate the whole
% method into two phases: (1) an one-time \textbf{compression}
% (\algref{a:compress}),
% and (2) an \textbf{evaluation} (\algref{a:evaluate}) for each $w$ instance.
% These algorithms are described in terms of binary tree traversals: 
% postorder \textbf{POST}, preorder \textbf{PRE},
% any order \textbf{ANY} and \textbf{LEAF} (only traverse leaf nodes).
% The computation that occurs in each tree
% node ($\alpha$ or $\beta$) is a task listed in 
% \tabref{tab:tasks}.
% 
% \begin{algorithm}[!t]
% \caption{{} \texttt{Compress}($K$)}
% \begin{algorithmic}
%   \STATE \texttt{\bf for each} randomize projection tree
%   \STATE \gap \texttt{\bf PRE} \texttt{SPLI($\alpha$)} \# random projection tree 
%   \STATE \gap \texttt{\bf LEAF} \texttt{ANN($\alpha$)} \#\textbf{RAW} on \texttt{SPLI}
%   \STATE \texttt{\bf PRE} \texttt{SPLI($\alpha$)} \# metric ball tree 
%   \STATE \texttt{NearNear()} \#\textbf{RAW} on \#\texttt{SPLI} 
%   \STATE \texttt{\bf ANY} \texttt{Kba($\alpha$)} \#\textbf{RAW} on \texttt{NearNear}
%   \STATE \texttt{\bf LEAF} \texttt{NearFar($\beta$,root)} \#\textbf{RAW} on \texttt{NearNear}
%   \STATE \texttt{\bf POST} \texttt{FarFar($\alpha$)} \#\textbf{RAW} on \texttt{NearFar}
%   \STATE \texttt{\bf POST} \texttt{SKEL($\alpha$)} \#\textbf{RAW} on \texttt{SPLI}
%   \STATE \texttt{\bf ANY} \texttt{COEF($\alpha$)} \#\textbf{RAW} on \texttt{SKEL}
%   \STATE \texttt{\bf ANY} \texttt{SKba($\alpha$)} \#\textbf{RAW} \texttt{FarFar}
%   and \texttt{SKEL}
% \end{algorithmic}
% \label{a:compress}
% \end{algorithm}
% 
% 
% \begin{table}[!t]
% \centering
% {
% \begin{tabular}{|rlr|}
% \hline 
% Task & Operations & \texttt{FLOPS} \\
% \hline 
% \texttt{SPLI($\alpha$)} & split $\alpha$ into $\lc$ and $\rc$ \algref{a:split} & $\lvert \alpha \rvert$ \\
% \hline 
% \texttt{ANN($\alpha$)} & update $\MA{N}_{\alpha}$ with \texttt{KNN($K_{\alpha\alpha}$)} & $dm^2$ \\ 
% \hline 
% \texttt{SKEL($\alpha$)} & $\sk{\alpha}$ in \algref{a:skeletonize} & $2s^3+2m^3$ \\ 
% \hline 
% \texttt{COEF($\alpha$)} & $P_{\sk{\alpha} \alpha}$ and $P_{\sk{\alpha} [\sk{\lc} \sk{\rc}]}$ in \algref{a:skeletonize} & $s^3$ \\ 
% \hline 
% \texttt{N2S($\alpha$)} & \texttt{\bf if} $\alpha$ is leaf \texttt{\bf then} $\sk{w_{\alpha}} = P_{\sk{\alpha}\alpha}w_{\alpha}$ & $2msr$ \\
%              & \texttt{\bf else} $\sk{w_{\alpha}} =
% P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}[ \sk{w_{\lc}}; \sk{w_{\rc}}]$ & $2s^2r$\\
% \hline
% \texttt{SKba($\beta$)}  & $\forall\alpha\in Far(\beta)$, $K_{\sk{\beta}\sk{\alpha}} = K(\sk{\beta}, \sk{\alpha})$ & $ds^2\lvert Far(\beta) \rvert$ \\ 
% \hline 
% \texttt{S2S($\beta$)} & $\sk{u_{\beta}} =
%   \sum_{\alpha\in Far(\beta)} K_{\sk{\beta}\sk{\alpha}}\sk{w_{\alpha}}$ & $2s^2r\lvert Far(\beta) \rvert$\\ 
% \hline 
% \texttt{S2N($\beta$)} & \texttt{\bf if} $\alpha$ is leaf \texttt{\bf then} $u_{\beta} = P_{\sk{\beta}\beta}^{T}\sk{u_{\beta}}$ & $2msr$ \\ 
%                       & \texttt{\bf else} $[\sk{u_{\lc}};\sk{u_{\rc}}] += P_{\sk{\beta}[\sk{\lc}\sk{\rc}]}^{T}\sk{u_{\beta}}$ & $2s^2r$ \\
% \hline
% \texttt{Kba($\beta$)}  & $\forall\alpha\in Near(\beta)$, $K_{\beta\alpha} = K(\beta, \alpha)$ & $dm^2\lvert Near(\beta) \rvert$ \\ 
% \hline  
% \texttt{L2L($\beta$)} & $u_{\beta} += \sum_{\alpha\in Near(\beta)}K_{\beta\alpha}w_{\alpha}$ & $2m^2r\lvert Near(\beta) \rvert$\\ 
% \hline 
% \end{tabular}
% }
% \caption{Tasks and their costs in \texttt{FLOPS}.
%   \texttt{SPLI} (tree splitting), \texttt{ANN} (all nearest-neighbor), \texttt{SKEL} (skeletonization), 
%   \texttt{COEF} (interpolation) \texttt{SKba} and 
%   \texttt{Kba} (caching submatrices) appear in the setup phase.
%   Interactions \texttt{N2S} (nodes to skeletons), \texttt{S2S} (skeletons to skeletons)
%   , \texttt{S2N} (skeletons to nodes) and \texttt{L2L} (leaves to leaves) appear in 
% the evaluation phase.}
% \label{tab:tasks}
% \end{table} 
% 
% 
% \textbf{Compression.}
% In this paper we apply a black-box geometry-oblivious heuristic
% to define \emph{distance} between pairs of rows (and columns).
% This \emph{distance} allows us to define neighbors $\MA{N}$ for
% each index, and partition $K$ with a metric ball tree~\cite{}.
% Given the capability of accessing any $K_{ij}$ element, 
% we first explain how such \emph{distance} is defined by only using
% raw elements from $K$; then we present the compression algorithm,
% which follows~\cite{} but in the flavor of \emph{out-of-order} using
% task scheduling.
% 
% 
% %\begin{enumerate}
% %\item hierarchical binary partitioning of the input matrix
% %\item a {\it distance} metric for neighbor sampling
% %\end{enumerate}
% %\input{hierarchical.tex}
% 
% 
% 
% Any symmetric positive-definite (SPD) matrix can be described as 
% a \emph{Gramian matrix} of some set of vectors $\{\phi_i\}$.
% Given a matrix $K$ (e.g. from a kernel function $K_{ij}=\MA{K}(x_i,x_j)$,
% where $x_{i} \in \mathbb{R}^{d}$) being symmetric 
% positive definite, we can assume that there exists a set of vectors 
% $\phi_i \in \mathcal{V}$ which define this matrix by an inner product,  
% $K_{ij}=\mathcal{K} (x_i,x_j)=\phi_i^{T}\phi_j$.
% Hence, we can define \emph{distance} $d_{ij}$ between $\phi_i$ and $\phi_j$
% in the Gramian space. We use two metrics:
% \begin{itemize}
% \item the $L^2$ distance $\|\phi_i-\phi_j\|_2^2=K_{ii}+K_{jj}-2K_{ij}$, or
% \item the $\sin{}$ similarity $1- \K_{ij}^2 / (K_{ii}K_{jj}) $.
% \end{itemize}
% These \emph{distances} define hierarchical subdivisions.
% 
% \begin{algorithm}[!t]
%   \caption{{} $[\lc,\rc]=\texttt{metricSplit}(\alpha)$}
% \begin{algorithmic}
%   \STATE $p = argmax( \{\sum_{j\in\texttt{c}}d_{ij} / \lvert \texttt{c} \rvert
%   \lvert i \in \alpha \})$
%   \STATE $q = argmax( \{ d_{ip} \lvert i \in \alpha \})$
%   \STATE $[\lc,\rc]=medianSplit(\{ d_{ip} - d_{iq} \lvert i \in \alpha\})$
% \end{algorithmic}
% \label{a:split}
% \end{algorithm}
% 
% 
% Starting from all indicies (\texttt{root}), we use a metric ball 
% tree to recursively partition indicies into two
% children $\lc$ and $\rc$. 
% This task is described as \texttt{SPLI($\alpha$)}
% in \tabref{tab:tasks} using \algref{a:split}. 
% Let's define an approximate centroid by $\hat{\phi_\alpha}= \frac{1}{\lvert \texttt{c}\rvert}\sum_{i\in\texttt{c}}\phi_{i}$,
% where $\texttt{c} \subset \alpha$ contains a constant number of samples, in order to avoid accessing $\MA{O}(N)$ entries.
% With this approximate centroid, we first find $p$ as the most far away
% index from the centroid in $\MA{O}(\lvert c \rvert\lvert\alpha\rvert)$, and we find $q$
% corresponding to $p$ in $\MA{O}(\lvert\alpha\rvert)$.
% 
% Next, we compute a \emph{distance} for each index $i$ towards $p$ and $q$, i.e. $d_{ip} - d_{iq}$. 
% Then we perform a median split on this metric $d_{ip} - d_{iq}$.
% This results in an even split, and $p$, $q$ will be in a different child.
% \texttt{SPLI($\alpha$)} stops when $\lvert \alpha \rvert \leq m$, a user defined leaf node size.
% %To avoid $\MA{O}(N^2)$ search on $d_{pq}$, an approximate centroid is defined as $\sum_{i\in\texttt{c}}\phi_{i} / \lvert \texttt{c} \rvert$, where $\texttt{c} \subset \alpha$ contains constant number of samples.
% 
% 
% The neighbors $\MA{N}$ are defined using the same metric $d_{ij}$.
% We employ an iterative neighbor search~\cite{} in \algref{a:compress} 
% that creates a binary 
% tree using randomized projection tree. That is, instead of searching for $p$ and
% $q$ in \algref{a:split}, we randomly select $p$ and $q$ from $\alpha$.
% In each iteration, exact neighbor search
% is only performed in the leaf level as \texttt{ANN($\alpha$)}
% shown in \tabref{tab:tasks}. 
% In this case, while searching for $k$ neighbors, we can restrict the
% candidate numbers to $\lvert \alpha \rvert$ (usually $2k$).
% Due to the randomness, these $2k$ candidates will be different 
% each time, and $\MA{N}$ may graduatelly converge\footnote{
% \scriptsize The convergence speed is affected by different factors; typically this is related to the intrinsic dimension of $K$.}.
% 
% 
% \textbf{Discussion.}
% Notice that in traditional FMM the \emph{distance} metric measures the 
% \emph{difficulty} of approximating the element. 
% 
% %This tree-like partition permutes $K$ into a hierarchical matrix whose 
% %off-diagonal blocks are potentially low-rank.
% %%We first define distance metrics for each column and row based on the symmetric factorization of $K$.
% %
% %For doing so, we consider a direction spanned by the two farthest 
% %points $\phi_\alpha$ and $\phi_\beta$ and split indices $i$ binary by
% %\begin{itemize}
% %\item[a.] a $L^2$ based splitting $<\phi_i,\phi_\alpha-\phi_\beta>$
% %\item[b.] a $d-1$-dimensional two-fold cone spanned in direction 
% %  $\phi_\alpha-\phi_\beta$, and its opposite direction 
% %  $\phi_\beta-\phi_\alpha$, 
% %  i.e. \\ $\frac{1}{\norm{\phi_i}}\lvert<\phi_i,\phi_\alpha-\phi_\beta>\rvert$
% %\end{itemize}
% 
% 
% 
% 
% %This tree-like partition permutes $K$ into a hierarchical matrix whose off-diagonal blocks are potentially low-rank.
% %We first define distance metrics for each column and row based on the symmetric factorization of $K$.
% %We then use these metrics to find neighbors and define the binary tree. 
% 
% %
% % define distance metrics here
% %
% 
% % section is reworded. please comment if unhappy
% %We then use these metrics to find neighbors; neighbors are computed 
% %with randomized projection tree based
% %algorithms. For each iteration, we select a random direction,
% %and split a tree node $\alpha$
% %into two children $\lc$ and $\rc$
% %\begin{itemize}
% %\item[a.] by a fictive orthogonal hyper-plane defined by the median
% % \item[b.] a fictive hyper-cone defined by a (roughly) equal-sized split 
% %\end{itemize}
% %An exhaustive neighbor search \texttt{ANN} is performed in each leaf node
% %$\alpha$ to update its neighbor list $\MA{N}_{\alpha}$.
% %When a pre-computed neighbor list is provided, this step is skipped.
% 
% % obsolete
% %The permutation for $K$ is computed with a ball tree. Given the distance metric, the two most far away points are select to form the projection direction. Again, a tree node $\alpha$ is split with the corresponding orthogonal hyper-plane. With this tree-based permutation, we can now compute the low-rank approximations for the off-diagonal blocks.
% 
% 
% \textbf{Low-rank approximations.}
% We now explain how skeleton $\sk{\alpha}$ is computed by the nested Interpolative Decomposition (ID) 
% in this work.
% Let $\alpha$ be the points in a tree node, and $S=\{1,...,N\}\backslash \alpha$
% be the set complement. The skeletonization of $\alpha$ is a rank-$s$
% approximation of its off-diagonal blocks $K_{S\alpha}$ using ID, 
% written as
% \begin{equation}
% K_{S\alpha} \approx K_{S\sk{\alpha}}P_{\sk{\alpha}\alpha}.
% \end{equation}
% Here $\sk{\alpha} \subset \alpha$ is the \emph{skeleton} of $\alpha$.
% $K_{S\sk{\alpha}}$ contains $s$ columns basis, and $P_{\sk{\alpha}\alpha} \in
% \mathbb{R}^{s\times \lvert \alpha \rvert}$ contains all interpolation
% coefficients.
% We use the first $s$ pivots of a rank-revealing QR factorization (\texttt{GEQP3}) 
% on $K_{S\sk{\alpha}}$ to select $\alpha$.
% With QR factorization of $K_{S\sk{\alpha}}$, we can compute
% $P_{\sk{\alpha}\alpha} = K_{S\sk{\alpha}}^{\dagger}K_{S\alpha}$ 
% with a triangular solver (\texttt{TRSM}).
% This scheme however results in $\bigO(d N^2\ppl)$ complexity for the
% overall factorization. We can turn it to a $\bigO(d \log N \ppl)$
% scheme by sampling a small subset $S'$ of $S$ and using it instead of
% $S$. With $\MA{N}(\alpha)$, we can perform importance sampling as shown 
% in~\cite{march-xiao-biros-e15}.
% The approximation rank $\ns$ is chosen such that
% $\sigma_{\ns+1}(K_{S' \alpha}) < \idtol$,
% where $\idtol$ is user-specified and $\sigma$ are the singular
% values estimated by the diagonal of the rank-revealing QR.
% 
% \begin{algorithm}[!t]
% \caption{{} [$\sk{\alpha}, P_{\sk{\alpha} \alpha}$]=\texttt{Skeleton}($\alpha$)}
% \begin{algorithmic}
%   \STATE \texttt{\bf if} $\alpha$ is leaf \texttt{\bf then return} [$\sk{\alpha}, P_{\sk{\alpha} \alpha}$] = {\tt ID}$(\alpha)$;
%   \STATE $[\sk{\lc},]=\texttt{Skeleton}(\lc)$; $[\sk{\rc},]=\texttt{Skeleton}(\rc)$;
%   \STATE \texttt{\bf return} [$\sk{\alpha}, P_{\sk{\alpha} [\sk{\lc} \sk{\rc}]
%   }$] = {\tt ID}($[\sk{\lc} \sk{\rc}]$);
% \end{algorithmic}
% \label{a:skeletonize}
% \end{algorithm}
% 
% \algref{a:skeletonize} computes skeletonization for all tree nodes with a 
% postorder traversal. As we have discussed in \secref{s:hier}, 
% for a non-leaf node $\alpha$, we use nested basis from children.
% Thus, instead of selecting 
% $\sk{\alpha}$ from $\alpha$, a greedy algorithm is used to only sub-select
% from children's skeleton $\sk{\lc}\cup\sk{\rc}$. Subsequently, 
% %instead of creating the whole coefficient matrix
% %$P_{\sk{\alpha}\alpha}$, we only compute the interpolation coefficients
% %$P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}$. 
% we have the \emph{telescoping} relationship shown in \eqref{e:telescoping}.
% Overall, \algref{a:skeletonize} has
% two tasks for each tree node $\alpha$ shown in \tabref{tab:tasks}: 
% (1) \texttt{SKEL($\alpha$)} selects $\sk{\alpha}$ (critical path) and
% (2) \texttt{COEF($\alpha$)} computes $P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}$ 
% (depending on $\sk{\alpha}$).
% Since the parallelism diminishes in \algref{a:skeletonize} during the 
% traversal, a proper schedule is required to improve the efficiency. 
% 
% \textbf{Evaluation.}
% While partial matrix-multiplication $u_{\beta} = K_{\beta\alpha}w_{\alpha}$
% can be interpreted as interaction between tree nodes $\beta$ and $\alpha$,
% We approximate $K_{\beta\alpha}$ with both column and row skeletons as
% $P_{\sk{\beta}\beta}^{T}K_{\sk{\beta}\sk{\alpha}}P_{\sk{\alpha}\alpha}$.
% Notice that due to the nested relation of $\alpha \subset \sk{\lc} \cup \sk{\rc}$,
% $P_{\sk{\alpha}\alpha}$ and $P_{\sk{\beta}\beta}$
% can be \emph{telescoped} recursively as
% \begin{equation}
% P_{\sk{\alpha}\alpha} =
% P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}
% \begin{bmatrix}
%   P_{\sk{\lc}\lc} & \\
%                   & P_{\sk{\rc}\rc} \\
% \end{bmatrix}.
% % \label{e:telescope}
% \end{equation}
% Recursive interpolation from both sides (left and right) is the key to achieve
% fast evaluation (less than quadratic). Still we need to first decide
% which pair of $\beta$ and $\alpha$ can be approximated and how to compute
% all pairs of interaction efficiently.
% 
% In \algref{a:nearfar} and \algref{a:farfar}, we decide which pair of
% interaction can be approximated and which cannot by traversing the tree
% top-down. 
% We collect all neighbors
% of a leaf node $\beta$ (including $\beta$ itself) named as $\MA{N}(\beta)$, 
% and we invoke \texttt{NearFar}($\beta$,\texttt{root}) for each $\beta$. 
% While traversing to $\alpha$,
% we say $\beta$ can prune $\alpha$ if none of $\MA{N}(\beta)$ appears in $\alpha$.
% We append $\alpha$ to $Far(\beta)$, which denotes all interactions that can be
% approximated with $\beta$. 
% Otherwise, we recurse to visit the children $\lc$ and $\rc$ of $\alpha$.
% While reaching the leaf level, if $\alpha$ still contains neighbors of $\beta$,
% then we append $\alpha$ to $Near(\beta)$, which denotes all interactions that
% cannot be approximated.
% \algref{a:nearfar} generates a list of prunable interactions for all leaf
% nodes. To generate prunable interaction lists for inner nodes, we merge
% two prunable lists from children to find the intersection.
% \algref{a:farfar} performs a post-order traversal, merging the far interaction
% lists from children, then removing duplications.
% 
% 
% % \begin{algorithm}
% % \caption{{} \texttt{Node2Skel}($\alpha$)}
% % \begin{algorithmic}
% % \STATE \texttt{\bf if} $\alpha$ is leaf \texttt{\bf then} $\sk{w_{\alpha}} = P_{\sk{\alpha}\alpha}w_{\alpha}$;
% % \texttt{\bf else} $\sk{w_{\alpha}} = P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}[ \sk{w_{\lc}}; \sk{w_{\rc}}]$;
% % \end{algorithmic}
% % \label{a:n2s}
% % \end{algorithm}
% % 
% % 
% % \begin{algorithm}
% % \caption{{} \texttt{Skel2Skel}()}
% % \begin{algorithmic}
% %   \STATE \texttt{\bf for each} $\beta$ \texttt{\bf do} $\sk{u_{\beta}} =
% %   \sum_{\alpha\in Far(\beta)} K_{\sk{\beta}\sk{\alpha}}\sk{w_{\alpha}}$;
% % \end{algorithmic}
% % \label{a:n2n}
% % \end{algorithm}
% % 
% % \begin{algorithm}
% % \caption{{} \texttt{Skel2Node}($\beta$)}
% % \begin{algorithmic}
% % \STATE \texttt{\bf if} $\beta$ is leaf \texttt{\bf then} $u_{\beta} = P_{\sk{\beta}\beta}^{T}\sk{u_{\beta}} + \sum_{\alpha\in Near(\beta)}K_{\beta\alpha}w_{\alpha}$;
% % \STATE \texttt{\bf else} $[\sk{u_{\lc}};\sk{u_{\rc}}] +=
% % P_{\sk{\beta}[\sk{\lc}\sk{\rc}]}^{T}\sk{u_{\beta}}$;
% % \end{algorithmic}
% % \label{a:n2s}
% % \end{algorithm}
% 
% 
% \begin{algorithm}
% \caption{{} \texttt{Evaluate}($u$,$w$)}
% \begin{algorithmic}
% \STATE \textbf{POST} \texttt{N2S($\alpha$)}
% \STATE \textbf{ANY} \texttt{S2S($\beta$)} \#\textbf{RAW} on \texttt{N2S}
% \STATE \textbf{PRE} \texttt{S2N($\beta$)} \#\textbf{RAW} on \texttt{S2S}
% \STATE \textbf{ANY} \texttt{L2L($\beta$)} \#\textbf{RAR} on \texttt{S2N}
% \end{algorithmic}
% \label{a:evaluate}
% \end{algorithm}
% 
% With the near and far interaction lists in hand, approximating the 
% matrix-multiplication of $K$ is described in \algref{a:evaluation}
% as a three-step process. 
% 
% \texttt{Node2Skel} performs a postorder traversal
% and computes the skeleton weight $\sk{w_{\alpha}}=P_{\sk{\alpha}\alpha}w_{\alpha}$ 
% for each tree node by multiplying the coefficient matrix on the left. 
% Recall from \eqref{e:telescope} that for a non-leaf node,
% $P_{\sk{\alpha}\alpha}$ can be \emph{telescoped} fast. 
% Thus, $\sk{w_{\alpha}}$ can be computed as
% $P_{\sk{\alpha}[\sk{\lc}\sk{\rc}]}[\sk{w_{\sk{\lc}}}\sk{w_{\sk{\rc}}}]$
% in the postorder traversal, because skeleton weights of both children have
% been computed. \texttt{Skel2Skel} traverses each node and compute the skeleton potentials
% $\sk{u_{\beta}} = \sum_{\alpha\in Far(\beta)}
% K_{\sk{\beta}\sk{\alpha}}\sk{w_{\alpha}}$.
% Finally \texttt{Skel2Node} performs a preorder traveral to accumulate
% all skeleton potentials. While traversing to leaf nodes, the aggregate
% potential is the summation of the skeleton potentials
% $P_{\sk{\beta}\beta}^{T}\sk{u_{\beta}}$
% and all direct interactions  
% $\sum_{\alpha\in Near(\beta)}K_{\beta\alpha}w_{\alpha}$.
% 
% \textbf{Complexity.} 
% While the worst case estimate of \algref{a:evalaute} is $\MA{O}(N^2)$
% (no approximation takes place), the best case appears when each 
% $Near(\alpha)$ only contains $\alpha$ itself.
% For a complete binary tree with $\MA{O}(N/m)$ leaf nodes, there are also 
% $\MA{O}(N/m)$ inner nodes.
% The cost for \texttt{Node2Skel} is $\MA{O}(sm(N/m)+2s^2(N/m))$.
% The cost for \texttt{Skel2Skel} is $\MA{O}(2s^2(N/m))$.
% Finally the cost for \texttt{Skel2Node} is
% $\MA{O(m^2(N/m)+sm(N/m)+2s^2(N/m))}$.
% When $s$ and $m$ are constant in $N$, the asympotoptic work 
% is $O(N)$ per right hand side.
% 


==> tables/dense_angle_budget1.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{7.284081E-01} & \num{1.700000}\% & \num{0.602000} & \num{0.360000} & \num{0.050000} & \num{0.002000} \\
\hline 
 K02N16384 & \num{16}& \accnum{1.250150E-05} & \num{2.100000}\% & \num{0.537000} & \num{0.350000} & \num{1.670000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{4.175128E-08} & \num{1.500000}\% & \num{0.450000} & \num{0.300000} & \num{0.040000} & \num{0.002000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.002797E-06} & \num{1.700000}\% & \num{0.491000} & \num{0.300000} & \num{1.000000} & \num{0.003000} \\
\hline 
 K05N16384 & \num{16}& \accnum{6.733814E-06} & \num{1.600000}\% & \num{0.498000} & \num{0.310000} & \num{1.300000} & \num{0.005000} \\
\hline 
 K06N16384 & \num{16}& \accnum{2.079063E-02} & \num{1.700000}\% & \num{0.493000} & \num{0.310000} & \num{1.190000} & \num{0.004000} \\
\hline 
 K07N16384 & \num{16}& \accnum{1.163419E-04} & \num{1.900000}\% & \num{0.492000} & \num{0.310000} & \num{1.240000} & \num{0.006000} \\
\hline 
 K08N16384 & \num{16}& \accnum{2.847905E-06} & \num{1.900000}\% & \num{0.497000} & \num{0.310000} & \num{1.180000} & \num{0.111000} \\
\hline 
 K09N16384 & \num{16}& \accnum{1.729423E-05} & \num{1.700000}\% & \num{0.484000} & \num{0.310000} & \num{1.200000} & \num{0.004000} \\
\hline 
 K10N16384 & \num{16}& \accnum{7.533478E-07} & \num{1.900000}\% & \num{0.495000} & \num{0.310000} & \num{1.090000} & \num{0.006000} \\
\hline 
 K12N16384 & \num{16}& \accnum{1.761285E-05} & \num{2.100000}\% & \num{0.427000} & \num{0.300000} & \num{1.050000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.362676E+00} & \num{2.100000}\% & \num{0.479000} & \num{0.310000} & \num{0.030000} & \num{0.002000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.287326E+00} & \num{2.100000}\% & \num{0.470000} & \num{0.310000} & \num{0.030000} & \num{0.002000} \\
\hline 
 K15N16384 & \num{16}& \accnum{1.126243E-01} & \num{1.500000}\% & \num{0.413000} & \num{0.310000} & \num{1.060000} & \num{0.003000} \\
\hline 
 K16N16384 & \num{16}& \accnum{4.373048E-01} & \num{1.700000}\% & \num{0.422000} & \num{0.300000} & \num{0.840000} & \num{0.011000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_angle_budget10.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{7.643909E-01} & \num{17.600000}\% & \num{0.696000} & \num{0.360000} & \num{0.110000} & \num{0.002000} \\
\hline 
 K02N16384 & \num{16}& \accnum{4.734992E-05} & \num{11.300000}\% & \num{0.428000} & \num{0.340000} & \num{1.680000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{4.203067E-08} & \num{16.600000}\% & \num{0.393000} & \num{0.300000} & \num{0.080000} & \num{0.002000} \\
\hline 
 K04N16384 & \num{16}& \accnum{1.993614E-06} & \num{14.200000}\% & \num{0.426000} & \num{0.310000} & \num{0.930000} & \num{0.005000} \\
\hline 
 K05N16384 & \num{16}& \accnum{4.590810E-06} & \num{13.900000}\% & \num{0.431000} & \num{0.310000} & \num{1.290000} & \num{0.005000} \\
\hline 
 K06N16384 & \num{16}& \accnum{2.459465E-02} & \num{13.800000}\% & \num{0.447000} & \num{0.310000} & \num{1.060000} & \num{0.005000} \\
\hline 
 K07N16384 & \num{16}& \accnum{1.766408E-04} & \num{15.800000}\% & \num{0.427000} & \num{0.310000} & \num{1.320000} & \num{0.005000} \\
\hline 
 K08N16384 & \num{16}& \accnum{3.037728E-06} & \num{15.300000}\% & \num{0.445000} & \num{0.310000} & \num{1.230000} & \num{0.006000} \\
\hline 
 K09N16384 & \num{16}& \accnum{1.755801E-05} & \num{13.900000}\% & \num{0.435000} & \num{0.310000} & \num{1.260000} & \num{0.005000} \\
\hline 
 K10N16384 & \num{16}& \accnum{7.572928E-07} & \num{15.500000}\% & \num{0.439000} & \num{0.310000} & \num{0.940000} & \num{0.006000} \\
\hline 
 K12N16384 & \num{16}& \accnum{1.172888E-05} & \num{7.700000}\% & \num{0.375000} & \num{0.310000} & \num{1.070000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.278301E+00} & \num{17.900000}\% & \num{0.423000} & \num{0.310000} & \num{0.090000} & \num{0.002000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.171085E+00} & \num{17.800000}\% & \num{0.432000} & \num{0.310000} & \num{0.090000} & \num{0.002000} \\
\hline 
 K15N16384 & \num{16}& \accnum{5.651690E-02} & \num{11.300000}\% & \num{0.403000} & \num{0.310000} & \num{1.140000} & \num{0.003000} \\
\hline 
 K16N16384 & \num{16}& \accnum{3.907982E-01} & \num{14.100000}\% & \num{0.422000} & \num{0.310000} & \num{0.820000} & \num{0.005000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_angle_hss.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{0}& \accnum{1.033845E+00} & \num{6.200000}\% & \num{0.000000} & \num{0.150000} & \num{0.390000} & \num{0.001000} \\
\hline 
 K02N16384 & \num{0}& \accnum{8.393876E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.800000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{0}& \accnum{4.495637E-08} & \num{6.200000}\% & \num{0.000000} & \num{0.150000} & \num{0.720000} & \num{0.001000} \\
\hline 
 K04N16384 & \num{0}& \accnum{2.373032E-06} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.460000} & \num{0.001000} \\
\hline 
 K05N16384 & \num{0}& \accnum{1.931233E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.290000} & \num{0.001000} \\
\hline 
 K06N16384 & \num{0}& \accnum{1.074791E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.960000} & \num{0.001000} \\
\hline 
 K07N16384 & \num{0}& \accnum{1.431807E-03} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.160000} & \num{0.001000} \\
\hline 
 K08N16384 & \num{0}& \accnum{1.352242E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.060000} & \num{0.001000} \\
\hline 
 K09N16384 & \num{0}& \accnum{6.023371E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.180000} & \num{0.001000} \\
\hline 
 K10N16384 & \num{0}& \accnum{9.298352E-07} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.990000} & \num{0.001000} \\
\hline 
 K12N16384 & \num{0}& \accnum{7.784573E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.620000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{0}& \accnum{8.376955E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.810000} & \num{0.001000} \\
\hline 
 K14N16384 & \num{0}& \accnum{9.741924E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.770000} & \num{0.001000} \\
\hline 
 K15N16384 & \num{0}& \accnum{2.913430E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.070000} & \num{0.001000} \\
\hline 
 K16N16384 & \num{0}& \accnum{5.395150E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.000000} & \num{0.001000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_angle_k16.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{7.721414E-01} & \num{54.800000}\% & \num{0.654000} & \num{0.320000} & \num{0.270000} & \num{0.002000} \\
\hline 
 K02N16384 & \num{16}& \accnum{2.160518E-06} & \num{11.800000}\% & \num{0.415000} & \num{0.320000} & \num{1.800000} & \num{0.002000} \\
\hline 
 K03N16384 & \num{16}& \accnum{4.174652E-08} & \num{45.000000}\% & \num{0.407000} & \num{0.290000} & \num{0.200000} & \num{0.002000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.048631E-06} & \num{51.000000}\% & \num{0.447000} & \num{0.310000} & \num{1.050000} & \num{0.005000} \\
\hline 
 K05N16384 & \num{16}& \accnum{7.013502E-06} & \num{49.700000}\% & \num{0.439000} & \num{0.290000} & \num{1.420000} & \num{0.005000} \\
\hline 
 K06N16384 & \num{16}& \accnum{1.968681E-02} & \num{45.600000}\% & \num{0.432000} & \num{0.290000} & \num{1.180000} & \num{0.005000} \\
\hline 
 K07N16384 & \num{16}& \accnum{1.922322E-04} & \num{70.000000}\% & \num{0.429000} & \num{0.300000} & \num{1.430000} & \num{0.006000} \\
\hline 
 K08N16384 & \num{16}& \accnum{3.067988E-06} & \num{68.400000}\% & \num{0.443000} & \num{0.290000} & \num{1.310000} & \num{0.006000} \\
\hline 
 K09N16384 & \num{16}& \accnum{1.977999E-05} & \num{48.900000}\% & \num{0.447000} & \num{0.290000} & \num{1.360000} & \num{0.004000} \\
\hline 
 K10N16384 & \num{16}& \accnum{7.570839E-07} & \num{61.500000}\% & \num{0.447000} & \num{0.300000} & \num{0.980000} & \num{0.006000} \\
\hline 
 K12N16384 & \num{16}& \accnum{6.087665E-05} & \num{7.400000}\% & \num{0.386000} & \num{0.300000} & \num{1.030000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{9.600817E-01} & \num{34.400000}\% & \num{0.429000} & \num{0.300000} & \num{0.160000} & \num{0.002000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.263432E+00} & \num{34.300000}\% & \num{0.443000} & \num{0.300000} & \num{0.150000} & \num{0.002000} \\
\hline 
 K15N16384 & \num{16}& \accnum{3.827181E-02} & \num{13.000000}\% & \num{0.414000} & \num{0.300000} & \num{1.150000} & \num{0.001000} \\
\hline 
 K16N16384 & \num{16}& \accnum{7.020218E-01} & \num{43.300000}\% & \num{0.429000} & \num{0.290000} & \num{0.810000} & \num{0.003000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_kerneldist_budget1.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{1.156279E+00} & \num{2.000000}\% & \num{0.644000} & \num{0.350000} & \num{0.050000} & \num{0.002000} \\
\hline 
 K02N16384 & \num{16}& \accnum{8.564398E-06} & \num{1.300000}\% & \num{0.401000} & \num{0.320000} & \num{1.720000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{4.701722E-08} & \num{2.000000}\% & \num{0.396000} & \num{0.310000} & \num{0.040000} & \num{0.002000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.207690E-06} & \num{1.600000}\% & \num{0.442000} & \num{0.290000} & \num{0.860000} & \num{0.004000} \\
\hline 
 K05N16384 & \num{16}& \accnum{7.440640E-06} & \num{1.500000}\% & \num{0.458000} & \num{0.300000} & \num{1.290000} & \num{0.004000} \\
\hline 
 K06N16384 & \num{16}& \accnum{1.411665E-02} & \num{1.700000}\% & \num{0.451000} & \num{0.300000} & \num{1.120000} & \num{0.005000} \\
\hline 
 K07N16384 & \num{16}& \accnum{3.641044E-04} & \num{2.100000}\% & \num{0.434000} & \num{0.300000} & \num{1.220000} & \num{0.005000} \\
\hline 
 K08N16384 & \num{16}& \accnum{2.738113E-06} & \num{2.100000}\% & \num{0.443000} & \num{0.310000} & \num{1.190000} & \num{0.006000} \\
\hline 
 K09N16384 & \num{16}& \accnum{2.425866E-05} & \num{1.600000}\% & \num{0.456000} & \num{0.300000} & \num{1.220000} & \num{0.003000} \\
\hline 
 K10N16384 & \num{16}& \accnum{7.660377E-07} & \num{2.100000}\% & \num{0.440000} & \num{0.300000} & \num{0.810000} & \num{0.005000} \\
\hline 
 K12N16384 & \num{16}& \accnum{2.085312E-04} & \num{1.200000}\% & \num{0.366000} & \num{0.300000} & \num{1.010000} & \num{0.000000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.649344E+00} & \num{1.400000}\% & \num{0.450000} & \num{0.300000} & \num{0.030000} & \num{0.000000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.355006E+00} & \num{1.400000}\% & \num{0.441000} & \num{0.300000} & \num{0.040000} & \num{0.001000} \\
\hline 
 K15N16384 & \num{16}& \accnum{1.418874E+00} & \num{2.100000}\% & \num{0.421000} & \num{0.300000} & \num{0.840000} & \num{0.004000} \\
\hline 
 K16N16384 & \num{16}& \accnum{1.295416E+00} & \num{2.100000}\% & \num{0.426000} & \num{0.300000} & \num{0.310000} & \num{0.007000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_kerneldist_budget10.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{1.119370E+00} & \num{18.100000}\% & \num{0.677000} & \num{0.370000} & \num{0.110000} & \num{0.002000} \\
\hline 
 K02N16384 & \num{16}& \accnum{2.842055E-06} & \num{1.700000}\% & \num{0.416000} & \num{0.340000} & \num{1.790000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{4.848862E-08} & \num{17.700000}\% & \num{0.394000} & \num{0.300000} & \num{0.090000} & \num{0.002000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.007957E-06} & \num{12.900000}\% & \num{0.475000} & \num{0.340000} & \num{0.930000} & \num{0.003000} \\
\hline 
 K05N16384 & \num{16}& \accnum{7.521480E-06} & \num{12.900000}\% & \num{0.439000} & \num{0.310000} & \num{1.320000} & \num{0.005000} \\
\hline 
 K06N16384 & \num{16}& \accnum{2.147991E-02} & \num{13.600000}\% & \num{0.433000} & \num{0.310000} & \num{1.150000} & \num{0.004000} \\
\hline 
 K07N16384 & \num{16}& \accnum{3.831132E-04} & \num{19.000000}\% & \num{0.451000} & \num{0.310000} & \num{1.410000} & \num{0.005000} \\
\hline 
 K08N16384 & \num{16}& \accnum{3.119662E-06} & \num{18.700000}\% & \num{0.424000} & \num{0.310000} & \num{1.290000} & \num{0.005000} \\
\hline 
 K09N16384 & \num{16}& \accnum{2.294723E-05} & \num{12.900000}\% & \num{0.446000} & \num{0.310000} & \num{1.340000} & \num{0.003000} \\
\hline 
 K10N16384 & \num{16}& \accnum{7.686730E-07} & \num{18.900000}\% & \num{0.439000} & \num{0.310000} & \num{0.830000} & \num{0.004000} \\
\hline 
 K12N16384 & \num{16}& \accnum{1.442071E-05} & \num{1.500000}\% & \num{0.373000} & \num{0.310000} & \num{1.070000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.867143E+00} & \num{4.900000}\% & \num{0.422000} & \num{0.310000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.640691E+00} & \num{4.900000}\% & \num{0.427000} & \num{0.310000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K15N16384 & \num{16}& \accnum{1.590483E+00} & \num{19.100000}\% & \num{0.430000} & \num{0.320000} & \num{0.850000} & \num{0.003000} \\
\hline 
 K16N16384 & \num{16}& \accnum{1.207052E+00} & \num{19.000000}\% & \num{0.431000} & \num{0.310000} & \num{0.440000} & \num{0.007000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_kerneldist_hss.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{0}& \accnum{1.167193E+00} & \num{6.200000}\% & \num{0.000000} & \num{0.150000} & \num{0.380000} & \num{0.001000} \\
\hline 
 K02N16384 & \num{0}& \accnum{1.039675E-04} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.740000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{0}& \accnum{4.898012E-08} & \num{6.200000}\% & \num{0.000000} & \num{0.150000} & \num{0.730000} & \num{0.001000} \\
\hline 
 K04N16384 & \num{0}& \accnum{2.450373E-06} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.330000} & \num{0.001000} \\
\hline 
 K05N16384 & \num{0}& \accnum{1.889322E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.220000} & \num{0.001000} \\
\hline 
 K06N16384 & \num{0}& \accnum{1.001707E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.930000} & \num{0.001000} \\
\hline 
 K07N16384 & \num{0}& \accnum{1.550451E-03} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.140000} & \num{0.001000} \\
\hline 
 K08N16384 & \num{0}& \accnum{1.168987E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.230000} & \num{0.001000} \\
\hline 
 K09N16384 & \num{0}& \accnum{5.312647E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.060000} & \num{0.001000} \\
\hline 
 K10N16384 & \num{0}& \accnum{9.477267E-07} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.960000} & \num{0.001000} \\
\hline 
 K12N16384 & \num{0}& \accnum{1.750477E-04} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{1.610000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{0}& \accnum{1.447855E+00} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.900000} & \num{0.001000} \\
\hline 
 K14N16384 & \num{0}& \accnum{1.425214E+00} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.710000} & \num{0.001000} \\
\hline 
 K15N16384 & \num{0}& \accnum{2.223244E+00} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.970000} & \num{0.001000} \\
\hline 
 K16N16384 & \num{0}& \accnum{9.506512E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.160000} & \num{0.940000} & \num{0.001000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_kerneldist_k16.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{1.159759E+00} & \num{55.000000}\% & \num{0.616000} & \num{0.370000} & \num{0.260000} & \num{0.002000} \\
\hline 
 K02N16384 & \num{16}& \accnum{5.854078E-06} & \num{1.700000}\% & \num{0.383000} & \num{0.320000} & \num{1.630000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{4.814530E-08} & \num{45.000000}\% & \num{0.401000} & \num{0.340000} & \num{0.210000} & \num{0.002000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.094125E-06} & \num{31.800000}\% & \num{0.466000} & \num{0.340000} & \num{0.980000} & \num{0.004000} \\
\hline 
 K05N16384 & \num{16}& \accnum{9.127756E-06} & \num{31.200000}\% & \num{0.433000} & \num{0.320000} & \num{1.330000} & \num{0.002000} \\
\hline 
 K06N16384 & \num{16}& \accnum{2.056182E-02} & \num{35.900000}\% & \num{0.438000} & \num{0.320000} & \num{1.220000} & \num{0.003000} \\
\hline 
 K07N16384 & \num{16}& \accnum{3.744029E-04} & \num{41.400000}\% & \num{0.437000} & \num{0.320000} & \num{1.390000} & \num{0.005000} \\
\hline 
 K08N16384 & \num{16}& \accnum{2.698770E-06} & \num{46.000000}\% & \num{0.442000} & \num{0.320000} & \num{1.290000} & \num{0.005000} \\
\hline 
 K09N16384 & \num{16}& \accnum{2.029909E-05} & \num{31.600000}\% & \num{0.436000} & \num{0.320000} & \num{1.490000} & \num{0.005000} \\
\hline 
 K10N16384 & \num{16}& \accnum{7.672375E-07} & \num{47.200000}\% & \num{0.424000} & \num{0.320000} & \num{0.890000} & \num{0.005000} \\
\hline 
 K12N16384 & \num{16}& \accnum{1.653503E-04} & \num{1.500000}\% & \num{0.381000} & \num{0.320000} & \num{1.030000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.177685E+00} & \num{4.900000}\% & \num{0.423000} & \num{0.320000} & \num{0.050000} & \num{0.000000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.745742E+00} & \num{4.800000}\% & \num{0.436000} & \num{0.320000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K15N16384 & \num{16}& \accnum{1.255908E+00} & \num{34.300000}\% & \num{0.426000} & \num{0.320000} & \num{0.830000} & \num{0.004000} \\
\hline 
 K16N16384 & \num{16}& \accnum{1.207530E+00} & \num{69.400000}\% & \num{0.423000} & \num{0.320000} & \num{0.350000} & \num{0.007000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_pointdist_budget1.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{5.961819E-08} & \num{1.300000}\% & \num{0.628000} & \num{0.090000} & \num{0.050000} & \num{0.000000} \\
\hline 
 K02N16384 & \num{16}& \accnum{1.704241E-06} & \num{1.300000}\% & \num{0.503000} & \num{0.080000} & \num{1.590000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{3.295138E-08} & \num{1.300000}\% & \num{0.440000} & \num{0.040000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.373921E-06} & \num{1.300000}\% & \num{0.433000} & \num{0.060000} & \num{1.180000} & \num{0.001000} \\
\hline 
 K05N16384 & \num{16}& \accnum{1.890602E-05} & \num{1.300000}\% & \num{0.434000} & \num{0.040000} & \num{1.260000} & \num{0.001000} \\
\hline 
 K06N16384 & \num{16}& \accnum{1.711800E-01} & \num{1.300000}\% & \num{0.422000} & \num{0.040000} & \num{1.090000} & \num{0.001000} \\
\hline 
 K07N16384 & \num{16}& \accnum{2.461710E-03} & \num{1.300000}\% & \num{0.441000} & \num{0.040000} & \num{1.320000} & \num{0.001000} \\
\hline 
 K08N16384 & \num{16}& \accnum{9.882976E-06} & \num{1.300000}\% & \num{0.425000} & \num{0.030000} & \num{1.140000} & \num{0.001000} \\
\hline 
 K09N16384 & \num{16}& \accnum{4.239003E-05} & \num{1.300000}\% & \num{0.419000} & \num{0.030000} & \num{1.210000} & \num{0.001000} \\
\hline 
 K10N16384 & \num{16}& \accnum{6.804214E-07} & \num{1.300000}\% & \num{0.430000} & \num{0.030000} & \num{0.870000} & \num{0.001000} \\
\hline 
 K12N16384 & \num{16}& \accnum{7.884804E-05} & \num{1.300000}\% & \num{0.394000} & \num{0.030000} & \num{1.100000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.106678E+00} & \num{1.300000}\% & \num{0.401000} & \num{0.040000} & \num{0.030000} & \num{0.000000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.113622E+00} & \num{1.300000}\% & \num{0.407000} & \num{0.030000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K15N16384 & \num{16}& \accnum{3.775960E-01} & \num{1.300000}\% & \num{0.404000} & \num{0.030000} & \num{0.900000} & \num{0.001000} \\
\hline 
 K16N16384 & \num{16}& \accnum{4.542683E-01} & \num{1.300000}\% & \num{0.397000} & \num{0.030000} & \num{0.410000} & \num{0.001000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_pointdist_budget10.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{5.961819E-08} & \num{2.300000}\% & \num{0.672000} & \num{0.090000} & \num{0.050000} & \num{0.000000} \\
\hline 
 K02N16384 & \num{16}& \accnum{1.704236E-06} & \num{2.300000}\% & \num{0.446000} & \num{0.050000} & \num{1.830000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{3.295138E-08} & \num{2.300000}\% & \num{0.338000} & \num{0.030000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.306653E-06} & \num{3.500000}\% & \num{0.376000} & \num{0.060000} & \num{1.150000} & \num{0.001000} \\
\hline 
 K05N16384 & \num{16}& \accnum{2.508772E-05} & \num{3.500000}\% & \num{0.373000} & \num{0.060000} & \num{1.320000} & \num{0.001000} \\
\hline 
 K06N16384 & \num{16}& \accnum{1.670733E-01} & \num{3.500000}\% & \num{0.369000} & \num{0.030000} & \num{1.030000} & \num{0.001000} \\
\hline 
 K07N16384 & \num{16}& \accnum{2.353217E-03} & \num{3.500000}\% & \num{0.353000} & \num{0.030000} & \num{1.210000} & \num{0.001000} \\
\hline 
 K08N16384 & \num{16}& \accnum{1.120513E-05} & \num{3.500000}\% & \num{0.362000} & \num{0.030000} & \num{1.200000} & \num{0.001000} \\
\hline 
 K09N16384 & \num{16}& \accnum{4.800565E-05} & \num{3.500000}\% & \num{0.364000} & \num{0.030000} & \num{1.210000} & \num{0.001000} \\
\hline 
 K10N16384 & \num{16}& \accnum{6.812538E-07} & \num{3.500000}\% & \num{0.428000} & \num{0.030000} & \num{0.850000} & \num{0.001000} \\
\hline 
 K12N16384 & \num{16}& \accnum{6.093608E-05} & \num{2.300000}\% & \num{0.343000} & \num{0.030000} & \num{1.100000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.108471E+00} & \num{2.300000}\% & \num{0.345000} & \num{0.030000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.117421E+00} & \num{2.300000}\% & \num{0.334000} & \num{0.030000} & \num{0.090000} & \num{0.000000} \\
\hline 
 K15N16384 & \num{16}& \accnum{3.536948E-01} & \num{2.300000}\% & \num{0.344000} & \num{0.040000} & \num{0.900000} & \num{0.001000} \\
\hline 
 K16N16384 & \num{16}& \accnum{4.563179E-01} & \num{2.300000}\% & \num{0.342000} & \num{0.030000} & \num{0.430000} & \num{0.001000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_pointdist_hss.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{0}& \accnum{3.243857E-02} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{0.290000} & \num{0.001000} \\
\hline 
 K02N16384 & \num{0}& \accnum{3.200495E-06} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.530000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{0}& \accnum{3.303678E-08} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{0.280000} & \num{0.001000} \\
\hline 
 K04N16384 & \num{0}& \accnum{2.405416E-06} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.370000} & \num{0.001000} \\
\hline 
 K05N16384 & \num{0}& \accnum{2.443407E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.250000} & \num{0.001000} \\
\hline 
 K06N16384 & \num{0}& \accnum{1.625561E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{0.980000} & \num{0.001000} \\
\hline 
 K07N16384 & \num{0}& \accnum{2.460025E-03} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.130000} & \num{0.001000} \\
\hline 
 K08N16384 & \num{0}& \accnum{1.092739E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.110000} & \num{0.001000} \\
\hline 
 K09N16384 & \num{0}& \accnum{4.571384E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.100000} & \num{0.001000} \\
\hline 
 K10N16384 & \num{0}& \accnum{9.217354E-07} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{0.960000} & \num{0.001000} \\
\hline 
 K12N16384 & \num{0}& \accnum{9.733571E-05} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.480000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{0}& \accnum{1.009218E+00} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{0.860000} & \num{0.001000} \\
\hline 
 K14N16384 & \num{0}& \accnum{9.375575E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{0.810000} & \num{0.001000} \\
\hline 
 K15N16384 & \num{0}& \accnum{3.375076E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.180000} & \num{0.001000} \\
\hline 
 K16N16384 & \num{0}& \accnum{3.481976E-01} & \num{6.200000}\% & \num{0.000000} & \num{0.010000} & \num{1.230000} & \num{0.001000} \\
 \bottomrule 
 \end{tabular}

==> tables/dense_pointdist_k16.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|llll} 
\toprule 
case  & k & error & $\%K$ & $t_{ANN}$ & $t_{setup}$ & $t_{skel}$ & $t_{eval}$ 
  \\\midrule 
\hline 
 K01N16384 & \num{16}& \accnum{5.961819E-08} & \num{2.300000}\% & \num{0.675000} & \num{0.090000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K02N16384 & \num{16}& \accnum{1.705087E-06} & \num{2.300000}\% & \num{0.516000} & \num{0.030000} & \num{1.660000} & \num{0.001000} \\
\hline 
 K03N16384 & \num{16}& \accnum{3.295138E-08} & \num{2.300000}\% & \num{0.418000} & \num{0.030000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K04N16384 & \num{16}& \accnum{2.351952E-06} & \num{3.500000}\% & \num{0.443000} & \num{0.030000} & \num{1.140000} & \num{0.001000} \\
\hline 
 K05N16384 & \num{16}& \accnum{2.041814E-05} & \num{3.500000}\% & \num{0.427000} & \num{0.040000} & \num{1.350000} & \num{0.001000} \\
\hline 
 K06N16384 & \num{16}& \accnum{1.584510E-01} & \num{3.500000}\% & \num{0.420000} & \num{0.040000} & \num{1.060000} & \num{0.001000} \\
\hline 
 K07N16384 & \num{16}& \accnum{2.301068E-03} & \num{3.500000}\% & \num{0.432000} & \num{0.060000} & \num{1.270000} & \num{0.001000} \\
\hline 
 K08N16384 & \num{16}& \accnum{1.195853E-05} & \num{3.500000}\% & \num{0.422000} & \num{0.040000} & \num{1.190000} & \num{0.001000} \\
\hline 
 K09N16384 & \num{16}& \accnum{4.533149E-05} & \num{3.500000}\% & \num{0.431000} & \num{0.040000} & \num{1.220000} & \num{0.001000} \\
\hline 
 K10N16384 & \num{16}& \accnum{6.823912E-07} & \num{3.500000}\% & \num{0.430000} & \num{0.030000} & \num{0.900000} & \num{0.001000} \\
\hline 
 K12N16384 & \num{16}& \accnum{6.837433E-05} & \num{2.300000}\% & \num{0.406000} & \num{0.040000} & \num{1.080000} & \num{0.001000} \\
\hline 
 K13N16384 & \num{16}& \accnum{1.091547E+00} & \num{2.300000}\% & \num{0.398000} & \num{0.030000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K14N16384 & \num{16}& \accnum{1.081877E+00} & \num{2.300000}\% & \num{0.412000} & \num{0.030000} & \num{0.040000} & \num{0.000000} \\
\hline 
 K15N16384 & \num{16}& \accnum{3.433667E-01} & \num{2.300000}\% & \num{0.403000} & \num{0.040000} & \num{0.990000} & \num{0.001000} \\
\hline 
 K16N16384 & \num{16}& \accnum{4.563017E-01} & \num{2.300000}\% & \num{0.396000} & \num{0.030000} & \num{0.430000} & \num{0.001000} \\
 \bottomrule 
 \end{tabular}

==> tables/otherSoftware.tex <==
\centering \scriptsize  
\begin{tabular}{l|lll|lll} 
\toprule 
& \multicolumn{3}{c}{HODLR} & \multicolumn{3}{c}{STRUMPACK}\\
case  & error & $t_{compr}$ & $t_{eval}$ & error & $t_{compr}$ & $t_{eval}$   \\
\midrule  
K01N16384 & \accnum{6.48E-006} & \num{1.98} & \num{30.05} & \accnum{4.75E-008} & \num{2.02792} & \num{0.275162} \\
K02N16384 & \accnum{0.291885} & \num{0.17} & \num{23.73} & \accnum{7.77E-005} & \num{0.612179} & \num{0.157362} \\
K03N16384 & \accnum{1.44E-016} & \num{0.19} & \num{13.84} & \accnum{-1} & \num{-1} & \num{-1} \\
K04N16384 & \accnum{0.00524736} & \num{0.42} & \num{30.81} & \accnum{0.000317365} & \num{1.75257} & \num{0.191612} \\
K05N16384 & \accnum{0.552039} & \num{1.78} & \num{45.13} & \accnum{0.0020794} & \num{4.51887} & \num{0.291494} \\
K06N16384 & \accnum{0.000187308} & \num{1196.18} & \num{371.48} & \accnum{7.94062} & \num{96.7403} & \num{0.641401} \\
K07N16384 & \accnum{2.86147} & \num{0.17} & \num{22.1} & \accnum{0.0609744} & \num{11.9258} & \num{0.348864} \\
K08N16384 & \accnum{0.0234354} & \num{0.27} & \num{25.4} & \accnum{0.00461083} & \num{6.90522} & \num{0.275341} \\
K09N16384 & \accnum{0.00701093} & \num{10.51} & \num{68.95} & \accnum{0.0127526} & \num{7.44834} & \num{0.294647} \\
K10N16384 & \accnum{0.832916} & \num{0.39} & \num{26.6} & \accnum{0.000128412} & \num{1.23641} & \num{0.183391} \\
K11N16384 & \accnum{9.41E-006} & \num{0.2} & \num{12.47} & \accnum{1.37E-007} & \num{0.493971} & \num{0.144428} \\
K12N16384 & \accnum{0.111046} & \num{0.17} & \num{22.54} & \accnum{7.00E-005} & \num{1.01366} & \num{0.182831} \\
K13N16384 & \accnum{4.05E-006} & \num{0.21} & \num{24.45} & \accnum{4.37E-007} & \num{0.81792} & \num{0.155076} \\
K14N16384 & \accnum{6.79E-006} & \num{0.22} & \num{24.52} & \accnum{5.78E-007} & \num{0.623684} & \num{0.156131} \\
K15N16384 & \accnum{0.741095} & \num{2.2} & \num{39.08} & \accnum{0.000368656} & \num{34.6946} & \num{0.497313} \\
K16N16384 & \accnum{3.65054} & \num{0.2} & \num{24.45} & \accnum{7.84E-005} & \num{29.3754} & \num{0.458744} \\ 
\bottomrule 
\end{tabular}


==> todo <==
2017/04/03 /******************************************************/
* More citations in the 'Background and significance' paragraph in the intro

2017/03/21 /******************************************************/
* FMM has a lot of evaluations, need to turn to treecode evaluation (requires symmetrizing nearest neighbors and leaf-leaf interactions); is the current TREECODE symmetric? Does it save evaluations?
leaf size:

* NANs removed? - DONE
* GPUs: are we using batched solves; are we using PASCAL (uniform memory); I'm mot sure we need scalability results for those machines, just performance for different parameters perhaps. 
* KNL: do we have an interesting story, do we use batched MKL (is it necssary?). What about MPI?
* Comparisons with other software: HOLDR, STRUMPACK, ASKIT (only for kernels) (does ASKIT support multiple RHS? if it is not, we need to normalize)
* Is ANN converging with for the angle,K-l2 metrics?
* cases that FMM provides more accuracy?  Make the case for FMM.

Batched 
* secondary:
- every run should have an ID so we can discuss it in the text
- all errors should be relative; are they?
- should not discuss sparse matrices, I don't see the reason in this paper and it will be confusing for the reader. 


2017/03/01 /******************************************************/
Summary: 
TODO: 
- Chenhan: 1.KNL and GPU implementation. - DONE
           2. error check in nearest-neighbors to at least have an indication of the error. - DONE
           3(?) May need to implement symmetric treecode;  - FMM H
- James: 1. point-based partitioning and nearest-neighbors for dense matrices only - DONE ?
         2. adaptive sampling - DONE?
- Severin: 1. runs for Gaussian matrix for k=0,1,2;   (also try smaller leaf sizes?)
           distance metrics: angle, matrix-l2, points-l2 
           2. create matlab script for latex tables.

WRITE UP: current format in sc17askit and assignments in paper is good. But coarser outline:
- James:    distance metrics;
- Severin: just dump result tables;
- Chenhan: Dynamic scheduling; KNL; GPU 

RESULTS:
- accuracy of method / comparison of different distance-metrics;
- scalability with matrix size
- dynamic-vs-static scheduling
- GPU-vs-CPU-vs-KNL


ISSUES: 
- FMM results in an excessive number of direct evaluations. Possible causes: metric used; bug; something in the implementation. If problem insists, implement symmetric tree-code and/or reduce number of evaluations by restricting direct evaluations to point-to-point as opposed to point-to-leaf. 
- Nearest neighbors are very inaccurate and seem to be useless; current implementation of having just 20 iterations without accuracy check (or even accuracy reporting) is problematic;
- adaptive row sampling is not implemented;
- adaptive rank selection is problematic, doesn't look at the norm of the entire  matrix

ISSUES: 
- Parameters: matrix type and size; # of nearest neighbors, max rank, adaptve-vs-nonadaptive, leaf size, distance criterios; treecode-vs-fmm
- Too many parameters for runs; for the paper fix rank; max rank = 1024; fix sampled rows. k=0,1,2
   Perhaps we can do the following:
   Report runs for all matrices for one or two parameter cases; and then report statistics or runs for certain matrices? 
- For graph matrices, I think we should report the case of k=0; for k=1, you get all the points in the graph and that's why we get good accuracy. Also, if the goal is to build an HSS matrix, the k=0 error will tell us whether this will work. 

THINGS NOT DISCUSSED: 
Comparison with other software (HOLDR and ASKIT are the best candidates).  Should definitely do if time permits.




2017/02/22 /******************************************************/
software to compare with:
- ASKIT (just for kernels)
These three packags below require reordering the matrix before passing it to them.
- https:/github.com/H2Lib/H2Lib
Seems to sfupport generic matrices through the new_pointer_amatrix() routine.
But dit is unclear how to create an hmatrix from an amatrix; all the constructions involve bie (integral equations) 
all examples are based on stencil or boundary integral equation problems; dh2compression seems to require some kind of tree structure.

- https://github.com/sivaramambikasaran/HODLR  
In the examples directory I don't see a way to specify the problem without introducing points.

- https://github.com/xantares/ahmed 
This seems to have an interface for sparse matrices, but there is no interface for dense matrices.
In principle, we could use the sparse-matrix interface for dense matrices but I don't think it will work and the reviewers may complain.
So basically no support for dense matrices; and the overall documentation is very poor.
This package supports MPI. 

Not sure if those are maintained.
?- https://bitbucket.org/poulson/dmhm   
Not maintained - seems to be only 2D or 3D
?- https://github.com/amiraa127/Dense_HODLR  
Unclear what's going on here. 

This is only for the inverse
http://portal.nersc.gov/project/sparse/strumpack/

2017/feb/10 /******************************************************/
[x] Large matrix interface
[x] JAMES:  OUT of core for large matrices: https://en.wikipedia.org/wiki/Mmap
 make sure your run on the new blades and that you use the local filesystem to store the matrix; a lot of filesystems on ronaldo are NFS mounted and they will be slow.

[x]JAMES: kernel evaluations using Bill's existing code
[ ]JAMES: kernel evaluations with gemm and a function that reports flops()

[x] CHENHAN: sparse matrices
https://snap.stanford.edu/data/
http://yifanhu.net/GALLERY/GRAPHS/search.html	
(I searched for symmetric matrices with more than 50K rows; by taking the square of those matrices and adding perhaps some small identity we can get positive definite versions)

[x] (CHENHAN) Replace omp task wait with omp task depend 

[ ]  (GEORGE) Create large Hessian and schur-Complement matrices. 

[x] Profiling costs: (SEVERIN)
     time and count kernel evaluations: time and count/estiamate flops/mops for different phases: finding which rows to sample, skeletonization, direct evaluations, 
Severin: please use the profiler and logger that Dhairya provided: it works really nice, I think. 
git clone https://github.com/dmalhotra/utils.git
         
[ ] (SEVERIN) Once profilinig is in, perform tests to various matrices -- need to identify all the major cost of the algorithm

[ ] Comparison with Nystrom methods, truncated randomized QR and the original ASKIT.

[ ] (CHENHAN) Nonsymmetric NN prunning list

todo - not necessary
[ ] GPU skeletonization and evaluation
[ ] finalize grouping and neighbor sampling  (frequency) and others
[ ] implement angle/cone neighbors, Severin (other splitters)
[ ] consider blocking matrix evaluations 
[x] add out of core capabilities for matrices 
[ ] sparse coordinates for kernel matrices
[ ] very hard: add support for sparse matrices (sparse ID?)

Current version supports: 
- FMM w/  direct evals + symmetric version
- TREE code done 
- Nearest sampling is done.
- Adaptive rank size done (but we need to motive criteria)
- matrix interface done  


2017/feb/02 /******************************************************/
Tree construction is sequential;
Nearest-neighbor is sequential; (leaf search is parallel)
Evaluation for one point, but no block evaluation
Symmetric lists are created but not in the evaluation
Block evaluation and FMM

[*] check accuracy
[ ] Replace omp task wait with omp task depend
[ ] Profiling costs and memory costs
[*] Correctness results for the matrices we have
[*] Interface for real matrices (different cases, try low-dimensional first to show performance, and Gaussian)



2017/01/18 : /******************************************************/
toso
severin:  runs double pass skeletonization: compares neighbors vs neighbors + uni sampling vs neighbors vs skeletons vs more neighbors
chenhan, james, severin: prepare outline for tree implementation


CODE
- Interface to matrix evaluation : 
getblocks( &vector<rows>, &vector<columns>)

- Tree construction
need to use randomization,  need to avoid excessive matrix evaluations. Avoid repeated calls to matrix interface, decide on rows based on depth of the tree.

- Make sure you create Morton-IDs in the tree construction

- Nearest neighbors (reuse rows for construction using randomization)

- Adaptive sampling

- Adaptive skeletonization

- Support for multiple Righ hand sides

- combine interaction lists to switch to BLAS2 evaluations

- Exploit asynchronous calculations as much as possible,

- Profiling/Instrumentation: for major phases of the algorithm estimate flops, other instructions (integer ops etc), memory reads and memory writes. 


-compress self-interactions and combine up the tree to create Nystrom approximation. 

-FMM? (probably no time)


External software.
ompUtils
smart pointers' Dhairya's work
profiler


Additional info for parallel tree construction:
You will need

https://github.com/dmalhotra/pvfmm.git/include/ and /src
ompUtils.{txx,h} has the parallel merge sort that you can use for the median, along with Chenhan's asynchronous tree construction.

The profiler should be profile.hpp (but it needs other stuff)
and in src/profile.cpp (unfortunately this requires MPI but perhaps we can remove it so we don't link to MPI)

The memory pointer (is like STL vector but with memory checks) is
mem_mgr.{hpp,txx}



ALGORITHMS
** Chair: Olivier Beaumont, Inria  - FMM hierarchical, fast direct solvers, scheduling
to cite: https://hal.inria.fr/hal-01361992/
\cite{agullo-beaumont16}
 (static scheduling is good with some augmentation)
Vice Chair: Judith C. Hill, Oak Ridge National Laboratory

* Emmanuel Agullo, INRIA -- scheduling/H-matrices
Guillaume Aupy, Inria - fault tolerance 
Wesley Bland, Intel Corporation -- MPI fault tolerance
Kate Clark, NVIDIA Corporation -- unclear no publications
Karen Devine, Sandia National Laboratories  -- graphs 
Ana Gainaru, Mellanox Technologies -- HPC MPI / IO
* Abdou Guermouche, Univ. Bordeaux  -- multifrontal solvers/StarPU/out-of-core/task scheduling
Thomas Herault, University of Tennessee -- fault tolerance
Mark Hoemmen, Sandia National Laboratories -- communication-avoiding (QR/LU,Krylov )
Mathias Jacquelin, Lawrence Berkeley National Laboratory -- LinLin: selected inversion (grigori crowd
Kamer Kaya, Sabancı University -- task scheduling and data placement
Christine Klymko, Lawrence Livermore National Laboratory -- graphs, clustering, linear algebra
Sarah Knepper, Intel Corporation  -- inverse problems (Naggy, optics)
* X. Sherry Li, Lawrence Berkeley National Laboratory -- STRUMPACK
* Hatem Ltaief, King Abdullah University of Science and Technology  -- Hierarchical matrices
Loris Marchal, CNRS & Univ. of Lyon -- scheduling / parallel cholesky factorization.
Anne-Cecile Orgerie, CNRS -- energy efficiency 
Cynthia Phillips, Sandia National Laboratories -- graphs clustering
Sanjay Rajopadhye, Colorado State University -- scheduling 
Krzysztof Rzadca, University of Warsaw -- networks 
Erik Saule, University of North Carolina, Charlotte -- data / task scheduling
Miroslav Stoyanov, Oak Ridge National Laboratory -- fluids, faults, UQ
Hari Sundar, University of Utah 
Harsh Vardhan, Google --  ? 
Frédéric Vivien, INRIA,  -- scheduling trees for multifrontal methods, out-orc-core, energy

